The MeerKAT 1.3 GHz Survey of the Small Magellanic Cloud

We present new radio continuum images and a source catalogue from the MeerKAT survey in the direction of the Small Magellanic Cloud (SMC). The observations, at a central frequency of 1.3 GHz across a bandwidth of 0.8 GHz, encompass a field of view ~7 x 7 degrees and result in images with resolution of 8 arcsec. The median broad-band Stokes I image Root Mean Squared noise value is ~11 microJy/beam. The catalogue produced from these images contains 108,330 point sources and 517 compact extended sources. We also describe a UHF (544-1088 MHz) single pointing observation. We report the detection of a new confirmed Supernova Remnant (SNR) (MCSNR J0100-7211) with an X-ray magnetar at its centre and 10 new SNR candidates. This is in addition to the detection of 21 previously confirmed SNRs and two previously noted SNR candidates. Our new SNR candidates have typical surface brightness an order of magnitude below those previously known, and on the whole they are larger. The high sensitivity of the MeerKAT survey also enabled us to detect the bright end of the SMC Planetary Nebulae (PNe) sample - point-like radio emission is associated with 38 of 102 optically known PNe, of which 19 are new detections. Lastly, we present the detection of three foreground radio stars amidst 11 circularly polarised sources, and a few examples of morphologically interesting background radio galaxies from which the radio ring galaxy ESO 029-G034 may represent a new type of radio object.

==> tables/MainTable.tex <==
\begin{table*}
\small
\begin{center}
\caption{Main catalogue.}
\label{tab:main}
\begin{tabular}{lllrrrrrrrrr}
\hline
Name          & RA (J2000)      &  DEC (J2000)       & Peak & Int &  a  & b & PA & $\alpha$ & $\chi^2$ & R$^2$ & n\\
              &                 &                    &(mJy/beam)  & (mJy)   & ('') & ('') & (deg) & & &  \\

\hline
  J001553-743313 & 00:15:52.77 & -74:33:13.1 & $0.132\pm0.025$ & $0.107\pm0.026$ & 8.1 & 6.4 & -80 & ... & ... & ... & ...\\
  J001614-743535 & 00:16:13.86 & -74:35:35.1 & $0.482\pm0.023$ & $0.545\pm0.031$ & 9.3 & 7.8 & 4 & $-1.08\pm0.37$ & 1.48 & 0.34 & 9\\
  J001615-743512 & 00:16:15.06 & -74:35:12.1 & $0.163\pm0.023$ & $0.197\pm0.035$ & 9.4 & 8.2 & -78 & ... & ... & ... & ...\\
  J001616-743321 & 00:16:16.04 & -74:33:20.6 & $0.146\pm0.021$ & $0.202\pm0.037$ & 9.6 & 9.2 & 12 & ... & ... & ... & ...\\
  J001621-742057 & 00:16:20.51 & -74:20:57.4 & $0.279\pm0.025$ & $0.289\pm0.030$ & 8.4 & 7.9 & -80 & $-0.41\pm0.78$ & 2.72 & -0.77 & 5\\
  J001625-742633 & 00:16:24.86 & -74:26:33.4 & $0.235\pm0.022$ & $0.243\pm0.026$ & 8.5 & 7.8 & 25 & $-2.17\pm1.14$ & ... & ... & 3\\
  J001633-742306 & 00:16:33.45 & -74:23:06.4 & $0.129\pm0.022$ & $0.149\pm0.032$ & 8.9 & 8.3 & 2 & ... & ... & ... & ...\\
  J001635-743112 & 00:16:34.76 & -74:31:12.3 & $0.108\pm0.022$ & $0.114\pm0.029$ & 8.6 & 7.9 & -2 & ... & ... & ... & ...\\
  J001637-743528 & 00:16:36.88 & -74:35:28.3 & $1.719\pm0.024$ & $1.872\pm0.031$ & 8.5 & 8.5 & 24 & $-0.81\pm0.11$ & 1.49 & 0.82 & 10\\
  J001638-743352 & 00:16:38.38 & -74:33:51.8 & $3.854\pm0.021$ & $4.145\pm0.026$ & 8.5 & 8.1 & -80 & $-1.15\pm0.03$ & 0.46 & 0.99 & 10\\

\hline
\end{tabular}
\end{center}
\end{table*}

\begin{table*}
\small
 \begin{center}
%\caption{Point source catalogue derived from our MeerKAT \ac{SMC} images. The catalogue at 1332\,MHz consists of \TOTALNUMBERCHZEROPEAKFLUX\ point sources. The full table is available in the online version of the article.}
\caption{Example of the MeerKAT broad-band (1332\,MHz) point source catalogue of \TOTALNUMBERCHZEROPEAKFLUX\ objects in the directions of the \ac{SMC} with its positions, integrated flux densities with associated uncertainty, and spectral index that is calculated using other sub-band flux densities. The columns provided are as follows: (1) Source name; (2 and 3) source position; (4 and 5) source peak and integrated flux density; (6 and 7) source extensions; (8) position angle; (9) spectral index fit to all available source components with the associated error; (10 and 11) reduced $\chi^2$ and R$^2$ values obtained in the spectral index fit (12) number of flux densities used in the spectral index fit. The full catalogue is provided through the VIZIER service and as supplementary material.}
\label{tab:main}
\begin{tabular}{lllccccccccccc}
\hline
Name          & RA (J2000)      &  DEC (J2000) & S$_{\rm peak\,1332\,MHz}$     & S$_{\rm int\,1332\,MHz}$       &  a        & b         & PA    & $\alpha\pm\Delta\alpha$ & $\chi^2$ & R$^2$ & n\\
              &                 &              &(mJy~beam$^{-1}$)& (mJy)         & (\arcsec) & (\arcsec) & (\D) & & &  \\
\hline
  J005049--724940 & 00:50:48.53 & --72:49:39.8 & 1.247$\pm$0.059 & 1.163$\pm$0.064 & --0.45$\pm$0.03 & 0.06 \\
  J004613--730704 & 00:46:13.22 & --73:07:04.5 & 3.485$\pm$0.062 & 4.137$\pm$0.086 & --0.82$\pm$0.02 & 0.09 \\
  J004516--730607 & 00:45:15.64 & --73:06:06.7 & 1.792$\pm$0.013 & 1.823$\pm$0.015 & --0.75$\pm$0.03 & 0.13 \\
  J011104--731155 & 01:11:03.95 & --73:11:55.1 & 1.473$\pm$0.015 & 1.522$\pm$0.018 & --0.92$\pm$0.03 & 0.19 \\
  J005242--723621 & 00:52:42.18 & --72:36:20.7 & 3.516$\pm$0.035 & 3.494$\pm$0.040 & --0.70$\pm$0.02 & 0.20 \\
  J004115--733600 & 00:41:14.79 & --73:36:00.0 & 2.712$\pm$0.042 & 2.827$\pm$0.050 & --0.75$\pm$0.02 & 0.20 \\
  J004852--731907 & 00:48:51.82 & --73:19:07.2 & 1.455$\pm$0.047 & 1.454$\pm$0.054 & --0.77$\pm$0.05 & 0.24 \\
  J012629--751001 & 01:26:29.01 & --75:10:00.7 & 1.527$\pm$0.015 & 1.563$\pm$0.017 & --0.78$\pm$0.03 & 0.27 \\
  J004347--750932 & 00:43:46.89 & --75:09:32.2 & 1.488$\pm$0.007 & 1.533$\pm$0.009 &   0.27$\pm$0.01 & 0.28 \\
  J004857--730954 & 00:48:57.16 & --73:09:53.6 & 1.369$\pm$0.027 & 2.395$\pm$0.055 & --0.02$\pm$0.04 & 0.33 \\
%
%  
%  J001553--743313 & 00:15:52.8 & --74:33:13 & $0.132\pm0.025$ & $0.107\pm0.026$ & 8.1 & 6.4 & --80 & ... & ... & ... & ...\\
%  J001614--743535 & 00:16:13.9 & --74:35:35 & $0.482\pm0.023$ & $0.545\pm0.031$ & 9.3 & 7.8 & 4    & $-1.08\pm0.37$ & 1.48 & 0.34 & 9\\
%  J001615--743512 & 00:16:15.1 & --74:35:12 & $0.163\pm0.023$ & $0.197\pm0.035$ & 9.4 & 8.2 & --78 & ... & ... & ... & ...\\
%  J001616--743321 & 00:16:16.0 & --74:33:21 & $0.146\pm0.021$ & $0.202\pm0.037$ & 9.6 & 9.2 & 12   & ... & ... & ... & ...\\
%  J001621--742057 & 00:16:20.5 & --74:20:57 & $0.279\pm0.025$ & $0.289\pm0.030$ & 8.4 & 7.9 & --80 & $-0.41\pm0.78$ & 2.72 & -0.77 & 5\\
%  J001625--742633 & 00:16:24.9 & --74:26:33 & $0.235\pm0.022$ & $0.243\pm0.026$ & 8.5 & 7.8 & 25   & $-2.17\pm1.14$ & ... & ... & 3\\
%  J001633--742306 & 00:16:33.5 & --74:23:06 & $0.129\pm0.022$ & $0.149\pm0.032$ & 8.9 & 8.3 & 2    & ... & ... & ... & ...\\
%  J001635--743112 & 00:16:34.8 & --74:31:12 & $0.108\pm0.022$ & $0.114\pm0.029$ & 8.6 & 7.9 & --2  & ... & ... & ... & ...\\
%  J001637--743528 & 00:16:36.9 & --74:35:28 & $1.719\pm0.024$ & $1.872\pm0.031$ & 8.5 & 8.5 & 24   & $-0.81\pm0.11$ & 1.49 & 0.82 & 10\\
%  J001638--743352 & 00:16:38.4 & --74:33:52 & $3.854\pm0.021$ & $4.145\pm0.026$ & 8.5 & 8.1 & --80 & $-1.15\pm0.03$ & 0.46 & 0.99 & 10\\
\hline
  \end{tabular}
 \end{center}
\end{table*}


==> tables/golden_sample.tex <==
\begin{table*}
 \small
 \begin{center}
\caption{Golden catalogue of radio star candidates}
 \label{tab:golden_star}
  \begin{tabular}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccc}
\hline
mainID & Name & RA2000 & DEC2000 & RAJ2000_deg & err_DRAJ2000 & DECJ2000_deg & err_DEJ2000 & ch0_local_rms & ch0_background & ch0_peak_flux & ch0_err_peak_flux & ch0_int_flux & ch0_err_int_flux & ch0_a & ch0_b & ch0_pa & ch0_residual_mean & ch0_residual_std & spindex & spindex_err & redchisq & adj_rsquare & no_points & ch2_local_rms & ch2_RA2000 & ch2_DEC2000 & ch2_ra & ch2_dec & ch2_peak_flux & ch2_err_peak_flux & ch2_int_flux & ch2_err_int_flux & ch2_Separation & ch3_local_rms & ch3_ra & ch3_dec & ch3_peak_flux & ch3_err_peak_flux & ch3_int_flux & ch3_err_int_flux & ch3_Separation & ch4_local_rms & ch4_ra & ch4_dec & ch4_peak_flux & ch4_err_peak_flux & ch4_int_flux & ch4_err_int_flux & ch4_Separation & ch5_local_rms & ch5_ra & ch5_dec & ch5_peak_flux & ch5_err_peak_flux & ch5_int_flux & ch5_err_int_flux & ch5_Separation & ch6_local_rms & ch6_ra & ch6_dec & ch6_peak_flux & ch6_err_peak_flux & ch6_int_flux & ch6_err_int_flux & ch6_Separation & ch7_local_rms & ch7_ra & ch7_dec & ch7_peak_flux & ch7_err_peak_flux & ch7_int_flux & ch7_err_int_flux & ch7_Separation & ch10_local_rms & ch10_ra & ch10_dec & ch10_peak_flux & ch10_err_peak_flux & ch10_int_flux & ch10_err_int_flux & ch10_Separation & ch11_local_rms & ch11_ra & ch11_dec & ch11_peak_flux & ch11_err_peak_flux & ch11_int_flux & ch11_err_int_flux & ch11_Separation & ch12_local_rms & ch12_ra & ch12_dec & ch12_peak_flux & ch12_err_peak_flux & ch12_int_flux & ch12_err_int_flux & ch12_Separation & ch13_local_rms & ch13_ra & ch13_dec & ch13_peak_flux & ch13_err_peak_flux & ch13_int_flux & ch13_err_int_flux & ch13_Separation & ch14_local_rms & ch14_ra & ch14_dec & ch14_peak_flux & ch14_err_peak_flux & ch14_int_flux & ch14_err_int_flux & ch14_Separation & ch15_local_rms & ch15_ra & ch15_dec & ch15_peak_flux & ch15_err_peak_flux & ch15_int_flux & ch15_err_int_flux & ch15_Separation & solution_id & designation & source_id & random_index & ref_epoch & ra & ra_error & dec & dec_error & parallax & parallax_error & parallax_over_error & pm & pmra & pmra_error & pmdec & pmdec_error & ra_dec_corr & ra_parallax_corr & ra_pmra_corr & ra_pmdec_corr & dec_parallax_corr & dec_pmra_corr & dec_pmdec_corr & parallax_pmra_corr & parallax_pmdec_corr & pmra_pmdec_corr & astrometric_n_obs_al & astrometric_n_obs_ac & astrometric_n_good_obs_al & astrometric_n_bad_obs_al & astrometric_gof_al & astrometric_chi2_al & astrometric_excess_noise & astrometric_excess_noise_sig & astrometric_params_solved & astrometric_primary_flag & nu_eff_used_in_astrometry & pseudocolour & pseudocolour_error & ra_pseudocolour_corr & dec_pseudocolour_corr & parallax_pseudocolour_corr & pmra_pseudocolour_corr & pmdec_pseudocolour_corr & astrometric_matched_transits & visibility_periods_used & astrometric_sigma5d_max & matched_transits & new_matched_transits & matched_transits_removed & ipd_gof_harmonic_amplitude & ipd_gof_harmonic_phase & ipd_frac_multi_peak & ipd_frac_odd_win & ruwe & scan_direction_strength_k1 & scan_direction_strength_k2 & scan_direction_strength_k3 & scan_direction_strength_k4 & scan_direction_mean_k1 & scan_direction_mean_k2 & scan_direction_mean_k3 & scan_direction_mean_k4 & duplicated_source & phot_g_n_obs & phot_g_mean_flux & phot_g_mean_flux_error & phot_g_mean_flux_over_error & phot_g_mean_mag & phot_bp_n_obs & phot_bp_mean_flux & phot_bp_mean_flux_error & phot_bp_mean_flux_over_error & phot_bp_mean_mag & phot_rp_n_obs & phot_rp_mean_flux & phot_rp_mean_flux_error & phot_rp_mean_flux_over_error & phot_rp_mean_mag & phot_bp_rp_excess_factor & phot_bp_n_contaminated_transits & phot_bp_n_blended_transits & phot_rp_n_contaminated_transits & phot_rp_n_blended_transits & phot_proc_mode & bp_rp & bp_g & g_rp & radial_velocity & radial_velocity_error & rv_method_used & rv_nb_transits & rv_nb_deblended_transits & rv_visibility_periods_used & rv_expected_sig_to_noise & rv_renormalised_gof & rv_chisq_pvalue & rv_time_duration & rv_amplitude_robust & rv_template_teff & rv_template_logg & rv_template_fe_h & rv_atm_param_origin & vbroad & vbroad_error & vbroad_nb_transits & grvs_mag & grvs_mag_error & grvs_mag_nb_transits & rvs_spec_sig_to_noise & phot_variable_flag & l & b & ecl_lon & ecl_lat & in_qso_candidates & in_galaxy_candidates & non_single_star & has_xp_continuous & has_xp_sampled & has_rvs & has_epoch_photometry & has_epoch_rv & has_mcmc_gspphot & has_mcmc_msc & in_andromeda_survey & classprob_dsc_combmod_quasar & classprob_dsc_combmod_galaxy & classprob_dsc_combmod_star & teff_gspphot & teff_gspphot_lower & teff_gspphot_upper & logg_gspphot & logg_gspphot_lower & logg_gspphot_upper & mh_gspphot & mh_gspphot_lower & mh_gspphot_upper & distance_gspphot & distance_gspphot_lower & distance_gspphot_upper & azero_gspphot & azero_gspphot_lower & azero_gspphot_upper & ag_gspphot & ag_gspphot_lower & ag_gspphot_upper & ebpminrp_gspphot & ebpminrp_gspphot_lower & ebpminrp_gspphot_upper & libname_gspphot & Separation & main_id & ra_x & dec_x & coo_err_maj & coo_err_min & coo_err_angle & nbref & ra_sexa & dec_sexa & coo_qual & coo_bibcode & main_type & other_types & radvel & radvel_err & redshift & redshift_err & sp_type & morph_type & plx & plx_err & pmra_x & pmdec_x & pm_err_maj & pm_err_min & pm_err_pa & size_maj & size_min & size_angle & B_x & V & R_x & J & H & K & u & g & r_xa & i & z & angDist \\
\hline
63250 & J004231-741155 & 00:42:31.07 & -74:11:55.0 & 10.629445075988766 & 6.732807e-05 & -74.19862365722658 & 8.74996e-05 & 0.00712317 & -0.0019419481 & 0.09185926 & 0.006944135 & 0.091234185 & 0.00793291 & 8.33285 & 7.631611 & 11.5960865 & 0.00016325839 & 0.002635834 & -1.23172 & 0.660008 & 7.62575 & 0.117822 & 5 & 0.02904731 & 00:42:31.09 & -74:11:55.8 & 10.62956 & -74.19883 & 0.1717978 & 0.027279316 & 0.25244534 & 0.049599998 & 0.7501551379628351 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.020555066 & 10.630027 & -74.198425 & 0.1189115 & 0.02011688 & 0.12860408 & 0.02624163 & 0.9138786448557589 & 0.020725518 & 10.629031 & -74.19882 & 0.13897747 & 0.020548351 & 0.12695622 & 0.021692 & 0.8213257714351424 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.021008827 & 10.628578 & -74.19861 & 0.10802395 & 0.020882344 & 0.108708814 & 0.028465167 & 0.85157931911385 & 1636148068921376768 & Gaia DR3 4685749263432487040 & 4685749263432487040 & 1160188389 & 2016.0 & 10.629195659365573 & 0.034324523 & -74.19869144226092 & 0.031908795 & 1.4482358761140017 & 0.037323635 & 38.802113 & 5.958813 & 3.406325630876241 & 0.054593917 & -4.889212740880988 & 0.042487644 & -0.15224643 & 0.16500852 & -0.106231675 & 0.019624438 & -0.290696 & 0.07333003 & 0.056241434 & -0.09397809 & -0.10640806 & -0.059339985 & 338 & 0 & 338 & 0 & -0.77270645 & 325.81366 & 0.0 & 0.0 & 31 & false & 1.4249643 &  &  &  &  &  &  &  & 39 & 27 & 0.0758439 & 47 & 13 & 0 & 0.011359617 & 65.850845 & 0 & 0 & 0.96921736 & 0.069304585 & 0.1625342 & 0.08991774 & 0.04883176 & -8.321131 & 21.962194 & 7.662702 & 36.705235 & false & 386 & 5987.077871481403 & 2.6513352 & 2258.137 & 16.24433 & 45 & 2326.7019537159977 & 5.929903 & 392.3676 & 16.92169 & 44 & 5232.928646645378 & 8.411672 & 622.1033 & 15.451034 & 1.2626578 & 0 & 1 & 0 & 0 & 0 & 1.4706564 & 0.67736053 & 0.79329586 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 303.76098940322214 & -42.91519463710077 & 308.4828666907253 & -64.5274163200273 & false & false & 0 & true & false & false & false & false & true & true & false & 1.0276925e-13 & 5.139892e-13 & 0.99992603 & 4496.0493 & 4489.3037 & 4501.73 & 4.5844 & 4.579 & 4.5895 & 0.1657 & 0.136 & 0.197 & 733.6618 & 730.6007 & 739.175 & 0.2326 & 0.2217 & 0.2425 & 0.1751 & 0.1668 & 0.1826 & 0.092 & 0.0877 & 0.096 & PHOENIX & 0.3872165848053219 & SSTISAGEMA J004231.00-741155.2 & 10.6291400623 & -74.1986697124 & 0.0 & 0.0 & 90.0 & 1 & 00 42 30.99361 & -74 11 55.2110 & A & 2020yCat.1350....0G & Star & *|IR|RB? &  &  &  &  &  &  & 1.4482 & 0.0373 & 3.406 & -4.889 & 0.055 & 0.042 & 90 &  &  &  & 17.73 & 16.57 &  & 14.482 & 13.869 & 13.705 &  &  &  &  &  & 0.376628 \\
102448 & J004403-743734 & 00:44:03.49 & -74:37:34.0 & 11.01452922821045 & 7.558388e-05 & -74.62609863281251 & 0.00010695931 & 0.007957531 & 0.0031086847 & 0.08631314 & 0.0078638345 & 0.081492744 & 0.008493732 & 8.49068 & 7.120909 & 19.593466 & 2.5623223e-05 & 0.004499452 & 1.32957 & 0.354152 & 0.501861 & 0.656791 & 4 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.01789297 & 11.0139065 & -74.626175 & 0.110847354 & 0.017818667 & 0.09017876 & 0.016909556 & 0.6547558299183193 & 0.015720075 & 11.014334 & -74.62614 & 0.096665464 & 0.015410722 & 0.10300742 & 0.019570576 & 0.23168063610231393 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.024624124 & 11.015511 & -74.62617 & 0.14648928 & 0.024505658 & 0.11877596 & 0.022879364 & 0.9686717686769105 & 1636148068921376768 & Gaia DR3 4685490259707560832 & 4685490259707560832 & 279690433 & 2016.0 & 11.01431433569211 & 0.012372453 & -74.626165947527 & 0.011690028 & 5.462415062794472 & 0.0133192055 & 410.1157 & 31.367102 & 30.991779892720313 & 0.014194363 & 4.837833881120612 & 0.016731681 & -0.17886803 & 0.27733007 & -0.25426343 & -0.10835597 & -0.1540398 & -0.023391427 & 0.015265212 & -0.09617285 & -0.1712177 & -0.08077919 & 323 & 323 & 322 & 1 & -3.6800318 & 807.7382 & 0.10766761 & 16.530867 & 31 & true & 1.5106277 &  &  &  &  &  &  &  & 37 & 27 & 0.023378834 & 44 & 16 & 1 & 0.009130585 & 115.610085 & 7 & 0 & 0.8564686 &  &  &  &  &  &  &  &  & false & 351 & 643813.7145732107 & 1150.1234 & 559.77795 & 11.165466 & 40 & 317966.21369018964 & 1808.0657 & 175.85988 & 11.58259 & 39 & 473773.0033274074 & 2160.2905 & 219.30986 & 10.5589695 & 1.2297645 & 0 & 16 & 0 & 16 & 0 & 1.0236206 & 0.4171238 & 0.6064968 & 10.342613 & 4.389282 & 1 & 20 & 4 & 18 & 64.642456 & 18.151564 & 0.0 & 897.0355 & 75.586075 & 6000.0 & 2.5 & 0.25 & 222 & 130.6595 & 39.32306 & 15 & 10.3077965 & 0.012809316 & 15 & 69.346344 & NOT_AVAILABLE & 303.5952401304983 & -42.49257688916182 & 307.66954710120245 & -64.79629409432931 & false & false & 0 & true & true & true & false & false & true & true & false & 1.0355536e-13 & 5.1725383e-13 & 0.99984825 & 5136.25 & 5117.991 & 5174.116 & 4.2639 & 4.2572 & 4.2858 & -0.5461 & -0.5687 & -0.487 & 181.7335 & 178.6733 & 182.5077 & 0.0991 & 0.086 & 0.1271 & 0.0804 & 0.0697 & 0.1033 & 0.0432 & 0.0374 & 0.0555 & MARCS & 0.293337084786247 & Flo 156 & 11.0137947835 & -74.6261874484 & 0.0 & 0.0 & 90.0 & 9 & 00 44 03.31075 & -74 37 34.2748 & A & 2020yCat.1350....0G & RotV* & *|IR|Ro*|V*|X & 10.6 & 2.6 & 3.54e-05 & 8.7e-06 & K0V &  & 5.4624 & 0.0133 & 30.992 & 4.838 & 0.014 & 0.017 & 90 &  &  &  & 12.12 & 11.565 &  & 9.872 & 9.398 & 9.309 &  &  &  &  &  & 0.763978 \\
57423 & J005205-744649 & 00:52:04.85 & -74:46:49.3 & 13.020203590393063 & 1.5101039e-05 & -74.78035736083984 & 1.3722898e-05 & 0.00667977 & -0.0030130227 & 0.07197463 & 0.006423335 & 0.07402789 & 0.006631154 & 8.276105 & 7.9579115 & 71.00843 & 0.0006800925 & 0.006185076 & 2.32444 & 0.287008 & 0.0865188 & 0.919684 & 4 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.016546872 & 13.021089 & -74.78037 & 0.088693455 & 0.015828284 & 0.07552179 & 0.013599644 & 0.8381994526085593 & 0.01395366 & 13.019991 & -74.780464 & 0.075834446 & 0.0134344315 & 0.08441466 & 0.0150101865 & 0.4338808803172716 & 0.013905825 & 13.019571 & -74.78006 & 0.08157951 & 0.013325067 & 0.09740282 & 0.015995054 & 1.2265718674066703 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4684816740118487936 & 4684816740118487936 & 1490864140 & 2016.0 & 13.020377590796047 & 0.0296105 & -74.78050128680196 & 0.027954256 & 4.829593555341997 & 0.03270989 & 147.64934 & 32.81383 & 32.511029357739275 & 0.042367462 & -4.447524424241904 & 0.03670703 & -0.016359862 & -0.00246129 & 0.06448876 & 0.015046879 & -0.05785448 & 0.024645092 & 0.053593453 & -0.13669032 & -0.23883748 & 0.01057501 & 311 & 0 & 311 & 0 & 1.2568315 & 350.76044 & 0.08979009 & 0.8449801 & 31 & false & 1.2925326 &  &  &  &  &  &  &  & 36 & 26 & 0.058722463 & 43 & 15 & 0 & 0.0189845 & 140.23659 & 0 & 0 & 1.0501248 & 0.056363396 & 0.08262188 & 0.056594826 & 0.1716504 & 26.775915 & 12.996627 & 20.386698 & 26.790737 & false & 353 & 8207.590866246619 & 6.814272 & 1204.4707 & 15.901828 & 39 & 1792.7111161114744 & 10.308232 & 173.91063 & 17.204767 & 40 & 9782.202045830232 & 15.034052 & 650.6697 & 14.771804 & 1.4102693 & 0 & 0 & 0 & 0 & 0 & 2.4329634 & 1.3029394 & 1.130024 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 302.87476932329565 & -42.3476772959775 & 307.8145401554182 & -65.34414367614544 & false & false & 0 & true & false & false & false & false & true & true & false & 1.13637784e-13 & 5.7128857e-13 & 0.99885 & 3607.1934 & 3598.87 & 3613.7144 & 4.73 & 4.7239 & 4.7359 & 0.0756 & 0.0621 & 0.0873 & 203.6236 & 201.0762 & 205.39 & 0.6713 & 0.6582 & 0.6825 & 0.4467 & 0.4379 & 0.4542 & 0.2765 & 0.271 & 0.281 & MARCS & 0.5293779956905833 & XMMU J005204.7-744649 & 13.019617 & -74.780412 & 1.1 & 1.1 & 90.0 & 1 & 00 52 04.708 & -74 46 49.48 & D & 2013A&A...558A...3S & Star & *|X &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.588113 \\
97185 & J005325-710243 & 00:53:25.46 & -71:02:42.7 & 13.356100082397457 & 7.0146685e-05 & -71.04519653320312 & 8.797163e-05 & 0.008436548 & -0.0011802738 & 0.11371068 & 0.007991765 & 0.136782 & 0.011125702 & 9.39063 & 8.203193 & 4.782241 & 4.0394934e-05 & 0.0030150164 & -1.01581 & 0.695699 & 2.21573 & 0.0389481 & 6 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0275294 & 13.35487 & -71.04498 & 0.16534492 & 0.026168054 & 0.24839622 & 0.050070364 & 1.6312571685602788 &  &  &  &  &  &  &  &  & 0.024875589 & 13.355791 & -71.04474 & 0.13098459 & 0.024306022 & 0.1864776 & 0.047460143 & 1.6870959040676725 & 0.0282084 & 13.355714 & -71.04518 & 0.14847668 & 0.028125573 & 0.13629921 & 0.032131102 & 0.4549797670850409 & 0.021442015 & 13.355797 & -71.04486 & 0.1313025 & 0.020907128 & 0.14207526 & 0.026847824 & 1.259455182491868 &  &  &  &  &  &  &  &  & 0.019151522 & 13.356201 & -71.04538 & 0.12839574 & 0.018215286 & 0.17375958 & 0.030757437 & 0.6696949534282862 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4689370676764568576 & 4689370676764568576 & 360936438 & 2016.0 & 13.35585143092205 & 0.0097778775 & -71.04517328736448 & 0.01020303 & 2.982694966471983 & 0.011509986 & 259.13977 & 37.37589 & 36.80401823534756 & 0.013292548 & 6.513164089040581 & 0.01443123 & -0.14608668 & 0.084578276 & -0.21167645 & -0.054118566 & -0.3227901 & -0.0548257 & 0.31651393 & -0.09303036 & -0.3069498 & -0.22618018 & 334 & 0 & 334 & 0 & -0.568504 & 323.00555 & 0.0 & 0.0 & 31 & false & 1.5056742 &  &  &  &  &  &  &  & 38 & 26 & 0.021660598 & 46 & 14 & 0 & 0.016735014 & 51.69943 & 0 & 0 & 0.976914 & 0.09062672 & 0.06917466 & 0.113947555 & 0.09424749 & 60.038944 & 35.6383 & 54.865795 & 31.739092 & false & 378 & 96304.5359084328 & 13.653024 & 7053.715 & 13.22825 & 44 & 46809.87054809196 & 25.556503 & 1831.6227 & 13.662699 & 44 & 70508.68466569265 & 27.080172 & 2603.7017 & 12.627289 & 1.2182038 & 0 & 1 & 0 & 1 & 0 & 1.0354099 & 0.4344492 & 0.60096073 & 68.94214 & 1.5841972 & 2 & 18 & 4 & 18 & 12.600628 &  &  & 896.71045 &  & 5000.0 & 4.0 & 0.0 & 111 &  &  &  & 12.3979845 & 0.050792962 & 14 &  & NOT_AVAILABLE & 302.69947326058906 & -46.08218059122561 & 315.7969642927746 & -63.84154272172898 & false & false & 0 & true & true & false & false & false & true & true & false & 1.0366049e-13 & 5.177789e-13 & 0.9998378 & 5292.7974 & 5283.1304 & 5301.5825 & 4.5744 & 4.567 & 4.5845 & 0.1056 & 0.0963 & 0.114 & 322.803 & 320.3268 & 324.2485 & 0.1887 & 0.1819 & 0.1949 & 0.1529 & 0.1474 & 0.1581 & 0.0809 & 0.0779 & 0.0837 & MARCS & 0.2816708203850726 & UCAC4 095-000849 & 13.3553478525 & -71.0452022341 & 0.0 & 0.0 & 90.0 & 1 & 00 53 25.28348 & -71 02 42.7280 & A & 2020yCat.1350....0G & Star & *|IR & 68.987 & 0.161 & 0.0002301 & 5e-07 &  &  & 2.9827 & 0.0115 & 36.804 & 6.513 & 0.013 & 0.014 & 90 &  &  &  & 14.291 & 13.454 & 13.298 & 11.937 & 11.51 & 11.405 &  & 13.84 & 13.188 & 12.957 &  & 0.860499 \\
2371 & J005611-724749 & 00:56:10.82 & -72:47:49.2 & 14.045101165771486 & 0.00013421956 & -72.79700469970703 & 0.0001178304 & 0.013951039 & -0.0118360715 & 0.13769472 & 0.011610579 & 0.30823532 & 0.031402253 & 12.86422 & 11.137031 & -87.80142 & 0.00037967565 & 0.0075713256 & -1.174 & 0.312209 & 0.883504 & 0.592486 & 9 & 0.03441382 & 00:56:10.77 & -72:47:49.5 & 14.044884 & -72.7971 & 0.17870401 & 0.028411416 & 0.5265894 & 0.11716726 & 0.4027742501649617 &  &  &  &  &  &  &  &  & 0.031843793 & 14.04523 & -72.79707 & 0.17314306 & 0.02829071 & 0.40130255 & 0.09390738 & 0.28265671625116123 & 0.028615164 & 14.044545 & -72.7972 & 0.17817736 & 0.025041424 & 0.36424917 & 0.064524084 & 0.9275733653542253 & 0.026576126 & 14.0463295 & -72.79717 & 0.1757007 & 0.024842054 & 0.2583565 & 0.046394072 & 1.440676057712501 & 0.02969344 & 14.045563 & -72.79686 & 0.17683624 & 0.027046204 & 0.2993232 & 0.055793524 & 0.7168394362392287 & 0.0235952 & 14.044554 & -72.79703 & 0.16368021 & 0.02154924 & 0.27398875 & 0.044869956 & 0.5886373217378048 & 0.02210505 & 14.04538 & -72.797386 & 0.123718694 & 0.019003449 & 0.29196155 & 0.06200796 & 1.4049332547960325 &  &  &  &  &  &  &  &  & 0.025763344 & 14.042876 & -72.79705 & 0.13353904 & 0.02393593 & 0.24702907 & 0.06574786 & 2.3746606411320816 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4685980435808569344 & 4685980435808569344 & 776256181 & 2016.0 & 14.044776170871598 & 0.28088343 & -72.79712818066898 & 0.22741583 & 0.16008522574811015 & 0.27734217 & 0.577212 & 5.8886833 & 4.9926282362864045 & 0.33623666 & -3.1225397438076987 & 0.27619535 & -0.24038053 & 0.20865497 & -0.28537127 & 0.101427495 & -0.115189664 & 0.19096203 & 0.0112541225 & -0.045231763 & -0.21037939 & -0.08882339 & 362 & 0 & 361 & 1 & 88.96303 & 12581.064 & 3.0429668 & 356.56512 & 95 & false &  & 1.5604631 & 0.064391024 & -0.06271011 & -0.022589633 & -0.13012825 & -0.016086197 & -0.009742895 & 41 & 28 & 0.48187542 & 46 & 17 & 0 & 0.15646565 & 116.51317 & 53 & 0 & 5.792057 & 0.10195164 & 0.21661703 & 0.03325873 & 0.098399885 & 21.160067 & 24.325762 & 18.424706 & 39.39803 & false & 320 & 2834.615066440731 & 9.2487135 & 306.4875 & 17.056131 & 44 & 3041.7728481674667 & 10.760414 & 282.68176 & 16.630726 & 43 & 1884.1753754792005 & 7.2081933 & 261.39355 & 16.560093 & 1.7377838 & 0 & 3 & 0 & 5 & 0 & 0.070632935 & -0.4254055 & 0.49603844 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 302.4419099587531 & -44.32661063760821 & 312.4073858018612 & -64.8215777180894 & false & false & 0 & true & false & false & false & false & false & true & false & 9.2155875e-05 & 5.1542255e-08 & 3.846109e-06 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.565591729109886 & OGLE SMC-SC7 181467 & 14.0445 & -72.7969166667 & 0.2 & 0.2 & 90.0 & 2 & 00 56 10.68 & -72 47 48.9 & C & 2003yCat.2246....0C & Star & *|IR &  &  &  &  & B0-5(IV) &  &  &  &  &  &  &  &  &  &  &  & 14.46 & 16.6 &  & 16.364 & 15.948 &  &  &  &  &  &  & 0.689751 \\
33010 & J010314-705059 & 01:03:14.46 & -70:50:59.0 & 15.810243606567383 & 5.6007622e-05 & -70.84971618652342 & 6.1532475e-05 & 0.009694956 & 0.0002679851 & 0.16938904 & 0.009369187 & 0.17885825 & 0.01135954 & 8.644241 & 7.8232493 & -12.348107 & 0.0009332205 & 0.0063701537 & -0.492014 & 0.490602 & 3.82517 & -0.135966 & 8 & 0.044503964 & 01:03:14.29 & -70:50:59.3 & 15.80956 & -70.84979 & 0.25016993 & 0.042696528 & 0.32470205 & 0.06861461 & 0.8529578403714809 &  &  &  &  &  &  &  &  & 0.030796818 & 15.809905 & -70.84947 & 0.1634522 & 0.03038698 & 0.17290947 & 0.040073793 & 0.9655755294247715 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0340029 & 15.810276 & -70.84958 & 0.24191664 & 0.032105017 & 0.30853093 & 0.049341727 & 0.49586555525740644 & 0.023265297 & 15.808921 & -70.84952 & 0.12617812 & 0.02223432 & 0.19634241 & 0.046688855 & 1.717616814304601 & 0.021293353 & 15.810296 & -70.84969 & 0.18967222 & 0.020583063 & 0.19621897 & 0.024660667 & 0.10308464508846309 & 0.02095233 & 15.810428 & -70.84973 & 0.18620233 & 0.019846423 & 0.22231862 & 0.027684314 & 0.22420168674518642 & 0.029201943 & 15.810278 & -70.84979 & 0.24979466 & 0.028722474 & 0.22577792 & 0.030111622 & 0.27763474062728105 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4690839693019667840 & 4690839693019667840 & 1287439949 & 2016.0 & 15.809988697453326 & 0.071264386 & -70.84976702193826 & 0.09816426 & 0.1278587405164408 & 0.07115657 & 1.796865 & 6.8321543 & 6.358557649895703 & 0.0952853 & -2.4994157039537743 & 0.14736763 & -0.4079757 & -0.15011552 & -0.6976761 & 0.34597915 & 0.04705137 & 0.33064166 & -0.5593279 & 0.14207563 & -0.40330628 & -0.26614377 & 150 & 142 & 145 & 5 & 32.121037 & 2811.1946 & 0.47921315 & 151.49646 & 95 & false &  & 1.447358 & 0.01711174 & -0.124194086 & -0.09427374 & 0.16431695 & 0.20402965 & 0.031941965 & 18 & 12 & 0.22087924 & 21 & 21 & 0 & 0.12244805 & 102.97513 & 86 & 0 & 3.4489076 &  &  &  &  &  &  &  &  & false & 140 & 162575.0126787922 & 260.32626 & 624.5048 & 12.659733 & 0 &  &  &  &  & 0 &  &  &  &  &  &  &  &  &  & 2 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 301.5328020165191 & -46.246408275389534 & 317.0555450301162 & -64.45697782310155 & false & false & 0 & false & false & false & false & false & false & false & false & -1.0 & -1.0 & -1.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.34819337946561735 & Cl* NGC  362     MV x2 c & 15.8104166667 & -70.8497222222 &  &  & 172.0 & 1 & 01 03 14.5 & -70 50 59 & D & 2007A&A...476.1261M & Star & * &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 10.45 &  & 9.64 &  &  &  &  &  & 0.196828 \\
41292 & J011322-724520 & 01:13:21.92 & -72:45:20.4 & 18.3413257598877 & 0.000122351 & -72.75566864013673 & 0.00010297056 & 0.009227459 & 0.0029242602 & 0.0816481 & 0.009061164 & 0.07835845 & 0.010094885 & 7.981863 & 7.6963263 & 86.82122 & 0.0001423544 & 0.00207005 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4687241365113885440 & 4687241365113885440 & 292192796 & 2016.0 & 18.341743535518162 & 0.12371507 & -72.75559373014961 & 0.12958573 & 1.6385854419068995 & 0.13912903 & 11.7774515 & 20.511833 & 16.967755959594264 & 0.15953474 & 11.525213546243602 & 0.17116627 & -0.01627616 & 0.23236513 & -0.14342335 & -0.039291356 & -0.13631193 & 0.000652179 & 0.078703664 & 0.02470864 & -0.1348878 & 0.07020431 & 404 & 0 & 403 & 1 & -1.7812768 & 410.87192 & 0.0 & 0.0 & 95 & false &  & 1.19521 & 0.03685293 & -0.01856744 & 0.08513559 & 0.05795672 & 0.03479158 & -0.13318938 & 46 & 28 & 0.24067675 & 51 & 17 & 0 & 0.0291817 & 80.523766 & 0 & 0 & 0.936634 & 0.03781804 & 0.07587554 & 0.07495281 & 0.07610158 & -91.8795 & 22.782785 & 38.866474 & 14.612518 & false & 433 & 578.6530045970635 & 0.98742515 & 586.02216 & 18.78132 & 45 & 149.37424132350083 & 5.0258474 & 29.721205 & 19.902853 & 44 & 789.9128373030768 & 7.529004 & 104.91598 & 17.503948 & 1.6232303 & 0 & 1 & 0 & 0 & 0 & 2.3989048 & 1.1215324 & 1.2773724 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 300.6649001928704 & -44.27600167386572 & 313.7144533739596 & -65.97219631540345 & false & false & 0 & false & false & false & false & false & false & false & false & 6.006601e-13 & 6.7705208e-12 & 0.999739 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.5104788337392092 & SSTISAGEMC J011322.00-724520.2 & 18.341489149 & -72.7556449532 & 0.0 & 0.0 & 90.0 & 1 & 01 13 21.95740 & -72 45 20.3218 & A & 2020yCat.1350....0G & Star & *|IR &  &  &  &  & M &  & 1.6386 & 0.1391 & 16.968 & 11.525 & 0.16 & 0.171 & 90 &  &  &  &  &  &  & 15.87 & 15.23 & 14.99 &  &  &  &  &  & 0.183745 \\
14116 & J011517-731143 & 01:15:16.56 & -73:11:43.2 & 18.81899070739746 & 6.502045e-05 & -73.19533538818361 & 5.3935975e-05 & 0.015121946 & 0.01253525 & 0.25323096 & 0.0149489585 & 0.24158293 & 0.01641437 & 7.983339 & 7.6494284 & 85.7914 & -0.00029687225 & 0.005246839 & -1.25751 & 0.270478 & 1.47965 & 0.620901 & 12 & 0.03757306 & 01:15:16.35 & -73:11:43.1 & 18.818106 & -73.1953 & 0.30252248 & 0.035846844 & 0.36218578 & 0.050290663 & 0.9312957330357802 & 0.054925155 & 18.819489 & -73.19549 & 0.31072482 & 0.052734174 & 0.44794953 & 0.10049365 & 0.7551166905271149 & 0.036455087 & 18.818542 & -73.19531 & 0.3490387 & 0.03489554 & 0.41538522 & 0.04907925 & 0.473733486794927 & 0.034890015 & 18.818691 & -73.195305 & 0.2934544 & 0.03418251 & 0.29224032 & 0.039593596 & 0.3304667576192775 & 0.034055173 & 18.818579 & -73.1954 & 0.32491672 & 0.032937936 & 0.36110204 & 0.042644937 & 0.48181293411743203 & 0.038317982 & 18.819365 & -73.195366 & 0.29575914 & 0.037941955 & 0.25363138 & 0.03698271 & 0.4043038556882267 & 0.033427063 & 18.818972 & -73.195366 & 0.28549635 & 0.033055495 & 0.2496561 & 0.033382274 & 0.11164240006504632 & 0.028165154 & 18.81877 & -73.19545 & 0.17677982 & 0.027588936 & 0.19087146 & 0.036055174 & 0.4719760061152311 & 0.0274879 & 18.8195 & -73.19525 & 0.2579168 & 0.026776496 & 0.25817496 & 0.030599192 & 0.6100983446678386 & 0.03405609 & 18.819475 & -73.19548 & 0.23905826 & 0.032971013 & 0.28539628 & 0.0486149 & 0.7256543162667715 &  &  &  &  &  &  &  &  & 0.033819 & 18.818254 & -73.19505 & 0.1940541 & 0.03374252 & 0.16606276 & 0.033956304 & 1.27275908495576 & 1636148068921376768 & Gaia DR3 4687166877510636032 & 4687166877510636032 & 304318451 & 2016.0 & 18.819092676892115 & 0.41833925 & -73.19526137931153 & 0.2834542 & 1.998383582462301 & 0.3284529 & 6.0842323 & 31.115095 & 22.15156507984593 & 0.53817654 & 21.85079553590774 & 0.40319175 & -0.41491598 & 0.09356812 & -0.2061393 & -0.19889347 & -0.022564538 & -0.1894438 & 0.42581767 & -0.20431845 & -0.16650183 & -0.40551046 & 200 & 0 & 200 & 0 & 1.902319 & 257.8012 & 1.117264 & 2.0749037 & 95 & false &  & 1.2342464 & 0.0845306 & -0.007908115 & -0.16030346 & -0.2561498 & 0.06993325 & 0.008403466 & 23 & 17 & 0.80592424 & 36 & 11 & 2 & 0.04033159 & 108.69663 & 0 & 63 & 1.0963416 & 0.1351147 & 0.5622147 & 0.07235883 & 0.22679284 & -173.38483 & 19.38757 & -49.77459 & -20.029963 & false & 221 & 379.87551456325104 & 1.3421843 & 283.02783 & 19.238264 & 0 &  &  &  &  & 0 &  &  &  &  &  &  &  &  &  & 2 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 300.54743338750217 & -43.82245015457656 & 312.8287273269352 & -66.2624547609141 & false & false & 0 & false & false & false & false & false & false & false & false & -1.0 & -1.0 & -1.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.27641089010875697 & XMMU J011516.1-731144 & 18.8188875 & -73.1954583333 & 0.19 & 0.17 & 42.0 & 2 & 01 15 16.533 & -73 11 43.65 & C & 2003yCat.2246....0C & Star & *|AG?|IR|X &  &  &  &  & M &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 16.4 & 15.53 & 15.17 &  &  &  &  &  & 0.464984 \\
108120 & J011705-722844 & 01:17:04.72 & -72:28:44.2 & 19.26967430114746 & 6.8554177e-06 & -72.47895050048828 & 5.595169e-06 & 0.007468951 & -0.002399937 & 1.3034515 & 0.007036373 & 1.6732854 & 0.010466455 & 9.285764 & 8.850377 & 84.02403 & 0.0015718959 & 0.03904704 & -0.702774 & 0.0376793 & 0.960201 & 0.967865 & 13 & 0.025024243 & 01:17:04.65 & -72:28:44.4 & 19.269384 & -72.47901 & 1.6513792 & 0.023339977 & 2.1749897 & 0.03550696 & 0.3834175639540552 & 0.03580544 & 19.269321 & -72.47901 & 1.5904242 & 0.033387817 & 2.065727 & 0.05013847 & 0.4410576932893356 & 0.022939593 & 19.26947 & -72.47897 & 1.5693884 & 0.021307835 & 2.048081 & 0.032262616 & 0.2360379897432297 & 0.021571144 & 19.26935 & -72.47898 & 1.5074356 & 0.020043222 & 1.9712856 & 0.030370506 & 0.3681945092042213 & 0.022408012 & 19.26948 & -72.478966 & 1.4130331 & 0.020672286 & 1.9054052 & 0.03229243 & 0.2178911077154126 & 0.027309006 & 19.269709 & -72.47892 & 1.3993027 & 0.025642632 & 1.7426319 & 0.03692104 & 0.11599345651592691 & 0.020831633 & 19.269808 & -72.47896 & 1.2395424 & 0.019395037 & 1.587115 & 0.028765079 & 0.14728672346074426 & 0.01631257 & 19.269714 & -72.47893 & 1.229676 & 0.015213008 & 1.5857877 & 0.022760255 & 0.09313353550229202 & 0.016305314 & 19.269854 & -72.47894 & 1.2071759 & 0.015276057 & 1.5134484 & 0.022175934 & 0.19624726528521835 & 0.0222661 & 19.269869 & -72.47891 & 1.1932572 & 0.021017132 & 1.4651166 & 0.029948296 & 0.25163160190817646 & 0.038939662 & 19.269918 & -72.478935 & 1.1070551 & 0.036043145 & 1.4777559 & 0.05539294 & 0.27024207296484565 & 0.02343105 & 19.269678 & -72.47892 & 1.1609956 & 0.021851962 & 1.4678415 & 0.032018505 & 0.10994104635992007 & 1636148068921376768 & Gaia DR3 4687350732164591104 & 4687350732164591104 & 1320607613 & 2016.0 & 19.269697530035913 & 0.15548316 & -72.47894937808042 & 0.12286878 & 1.1121822185579038 & 0.14173618 & 7.846848 & 6.540076 & -5.870731083765609 & 0.19558413 & 2.8822056617967737 & 0.16566159 & -0.17680062 & 0.1923474 & -0.28135428 & -0.074692115 & -0.11219973 & -0.06644848 & 0.19888043 & -0.030995645 & -0.100331895 & -0.21091248 & 369 & 0 & 368 & 1 & 0.069744036 & 406.7182 & 0.0 & 0.0 & 95 & false &  & 1.250421 & 0.039909728 & 0.12431029 & 0.15717064 & 0.0603647 & -0.023321116 & -0.008003481 & 43 & 28 & 0.2849602 & 45 & 16 & 0 & 0.022747433 & 76.91217 & 0 & 0 & 1.0016717 & 0.09826624 & 0.19202264 & 0.013889844 & 0.064279154 & 1.4414247 & 26.847172 & 19.15532 & -42.842033 & false & 372 & 603.0295111956946 & 1.1486365 & 524.996 & 18.73652 & 41 & 156.99054540620327 & 5.630433 & 27.8825 & 19.848858 & 41 & 740.9238463486594 & 5.7577963 & 128.68184 & 17.573462 & 1.4890057 & 0 & 2 & 0 & 0 & 0 & 2.2753963 & 1.1123371 & 1.1630592 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 300.23019460421506 & -44.514546909874646 & 314.60176455048554 & -66.12593542557732 & false & false & 0 & false & false & false & false & false & false & false & false & 2.0957459e-13 & 7.1800817e-13 & 0.9999107 & 3585.6238 & 3565.9658 & 3615.9014 & 4.289 & 4.2243 & 4.3565 & -0.1263 & -0.2232 & -0.026 & 1376.3787 & 1260.1855 & 1535.112 & 0.465 & 0.4034 & 0.5261 & 0.3111 & 0.2696 & 0.3522 & 0.1926 & 0.1676 & 0.2177 & MARCS & 0.03787274701586817 & SSTISAGEMA J011704.74-722844.1 & 19.2697841988 & -72.4789621879 & 0.0 & 0.0 & 90.0 & 1 & 01 17 04.74821 & -72 28 44.2639 & A & 2020yCat.1350....0G & Star & *|IR|RB? &  &  &  &  &  &  & 1.1122 & 0.1417 & -5.871 & 2.882 & 0.196 & 0.166 & 90 &  &  &  & 20.95 & 19.62 &  & 16.147 & 15.516 & 15.221 &  &  &  &  &  & 0.1425 \\
73060 & J011710-702150 & 01:17:09.72 & -70:21:49.7 & 19.29049301147461 & 0.0002852329 & -70.36381530761719 & 0.00022104605 & 0.009025444 & -0.0009900233 & 0.04648672 & 0.008922261 & 0.054136567 & 0.01411153 & 8.891102 & 8.3939495 & 83.907745 & 0.00018452061 & 0.0006424307 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4690959294964458880 & 4690959294964458880 & 76882503 & 2016.0 & 19.290799448319948 & 0.060681928 & -70.36368390724377 & 0.053701095 & 1.561043295933881 & 0.061360437 & 25.44055 & 33.214878 & 26.999543789278125 & 0.07608011 & 19.345615370554363 & 0.073836885 & 0.0007689296 & 0.24637249 & -0.3197272 & -0.03318037 & 0.06083207 & 0.0019496463 & 0.24167101 & -0.03243818 & -0.0033673365 & 0.055382982 & 379 & 0 & 376 & 3 & 0.14059025 & 391.90762 & 0.0 & 0.0 & 31 & false & 1.3607813 &  &  &  &  &  &  &  & 44 & 28 & 0.10906745 & 50 & 18 & 0 & 0.018561488 & 94.922485 & 0 & 0 & 1.0042658 & 0.07624971 & 0.092767574 & 0.059172176 & 0.030736916 & -95.939995 & 7.26976 & -55.365505 & -10.060498 & false & 402 & 2102.93687297207 & 1.7404815 & 1208.25 & 17.3803 & 47 & 663.5870734615139 & 9.013299 & 73.62311 & 18.283798 & 42 & 2083.407147808683 & 9.700674 & 214.76932 & 16.45096 & 1.3062657 & 0 & 28 & 0 & 28 & 0 & 1.832838 & 0.9034977 & 0.92934036 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 299.79101829736743 & -46.607364852716415 & 319.30326900852015 & -65.26956203217152 & false & false & 0 & true & false & false & false & false & true & true & false & 1.04428713e-13 & 5.2250733e-13 & 0.99976176 & 3659.4114 & 3649.667 & 3680.035 & 4.4101 & 4.4024 & 4.4326 & -1.134 & -1.1701 & -1.0651 & 558.186 & 545.0225 & 586.7952 & 0.0427 & 0.0206 & 0.0767 & 0.0302 & 0.0146 & 0.0543 & 0.0164 & 0.0079 & 0.0295 & PHOENIX & 0.5683496602427005 & SSTISAGEMA J011709.71-702149.4 & 19.2904423617 & -70.3637698874 & 0.0 & 0.0 & 90.0 & 1 & 01 17 09.70617 & -70 21 49.5716 & A & 2020yCat.1350....0G & Star & *|IR|RB? &  &  &  &  &  &  & 1.561 & 0.0614 & 27.0 & 19.346 & 0.076 & 0.074 & 90 &  &  &  &  &  &  & 15.284 & 14.588 & 14.507 &  &  &  &  &  & 0.146117 \\
74414 & J012711-701022 & 01:27:10.58 & -70:10:22.5 & 21.794065475463867 & 0.00022926503 & -70.17290496826172 & 0.00015861778 & 0.010541261 & -0.0022406825 & 0.064230636 & 0.00974787 & 0.09889829 & 0.018616099 & 10.575031 & 9.336358 & -87.25181 & -0.0005688477 & 0.0036990598 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4691120446431145088 & 4691120446431145088 & 1346509473 & 2016.0 & 21.79404897762819 & 0.06420532 & -70.17283296035956 & 0.055746477 & 0.4133221658854536 & 0.066142514 & 6.2489634 & 10.324254 & 4.022415287205852 & 0.091147356 & -9.508437715487478 & 0.07209633 & 0.030814085 & -0.106000826 & -0.38929418 & -0.008496812 & -0.20564032 & -0.019260807 & 0.044946693 & -0.027043736 & -0.26156265 & 0.05259128 & 330 & 0 & 330 & 0 & 0.21511512 & 343.0739 & 0.0 & 0.0 & 31 & false & 1.5469518 &  &  &  &  &  &  &  & 38 & 25 & 0.12931679 & 42 & 15 & 0 & 0.013471638 & 71.31412 & 0 & 0 & 1.007421 & 0.1453205 & 0.105606265 & 0.029303502 & 0.13186364 & 63.844727 & -5.5069904 & 42.9997 & 22.42199 & false & 341 & 2119.3092128686294 & 1.686015 & 1256.993 & 17.371881 & 39 & 1093.5511035688482 & 11.431374 & 95.66227 & 17.741444 & 38 & 1439.3662224146785 & 11.389935 & 126.37177 & 16.852467 & 1.1951617 & 0 & 1 & 0 & 1 & 0 & 0.88897705 & 0.36956215 & 0.5194149 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 298.5308902004629 & -46.64883390945984 & 320.60394387258424 & -65.94936619844896 & false & false & 0 & true & false & false & false & false & true & true & false & 6.2761296e-11 & 5.1017236e-13 & 0.99999106 & 5443.682 & 5401.1177 & 5520.9214 & 4.7082 & 4.6819 & 4.7353 & -2.1308 & -2.3033 & -1.9093 & 1696.4006 & 1642.9707 & 1768.7574 & 0.0408 & 0.0068 & 0.0983 & 0.0339 & 0.0056 & 0.0821 & 0.0185 & 0.0031 & 0.045 & MARCS & 0.30424868153133955 & [MCR2016] VMC-SMC-CEP 076 & 21.7939962707 & -70.1727907006 & 0.0 & 0.0 & 90.0 & 1 & 01 27 10.55910 & -70 10 22.0465 & A & 2020yCat.1350....0G & Cepheid & *|Ce* &  &  &  &  &  &  & 0.4133 & 0.0661 & 4.022 & -9.508 & 0.091 & 0.072 & 90 &  &  &  &  &  &  &  &  & 15.741 &  &  &  &  &  & 0.465772 \\
56668 & J002741-744049 & 00:27:41.09 & -74:40:48.9 & 6.921220779418942 & 9.152024e-05 & -74.68025970458984 & 0.00015213118 & 0.0094253635 & 0.0018937908 & 0.078049555 & 0.009064368 & 0.08357028 & 0.011257376 & 9.026902 & 7.6004972 & 1.0868177 & -0.00037632772 & 0.0021308395 & 4.24277 & 3.63316 &  &  & 2 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.019693151 & 6.921507 & -74.680504 & 0.103633694 & 0.019388873 & 0.114266515 & 0.026286706 & 0.9200684991488477 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4685345467763983104 & 4685345467763983104 & 834314489 & 2016.0 & 6.920807102493512 & 0.35841277 & -74.68015269522286 & 0.3234577 & 4.401071577979246 & 0.37652925 & 11.688525 & 16.532436 & 15.188555535461843 & 0.5424903 & 6.529106856405851 & 0.49106938 & -0.16489105 & -0.033130117 & -0.031120902 & 0.025082653 & -0.12253893 & 0.06406738 & 0.12574339 & -0.25854528 & 0.036828205 & -0.17050284 & 333 & 0 & 331 & 2 & 4.0266623 & 468.55106 & 1.8947598 & 3.5233297 & 95 & false &  & 1.2667918 & 0.113111936 & 0.084945805 & 0.14696744 & -0.0077037686 & 0.030214919 & -0.026549336 & 38 & 24 & 0.7849998 & 46 & 13 & 0 & 0.020327877 & 132.31561 & 0 & 0 & 1.1609478 & 0.123201355 & 0.1778039 & 0.0864663 & 0.12773797 & 8.734751 & 28.224342 & 46.918747 & -40.101074 & false & 389 & 206.5738592176803 & 0.81811845 & 252.49872 & 19.89968 & 26 & 52.80370232757853 & 6.001477 & 8.798451 & 21.031881 & 43 & 295.18300555859724 & 6.4950175 & 45.44761 & 18.572668 & 1.6845632 & 0 & 0 & 0 & 0 & 0 & 2.4592133 & 1.1322021 & 1.3270111 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 305.051678787898 & -42.350185290729726 & 306.50160302458727 & -63.83709722248009 & false & false & 0 & false & false & false & false & false & false & false & false & 2.6351409e-11 & 7.3765527e-09 & 0.99998236 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.5180230969449541 & 0.0 & 0.0 & 0.0 &  &  & 0.0 & 0 & 0.0 & 0.0 & 0 &  & 0.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0 \\
56514 & J003329-713246 & 00:33:29.25 & -71:32:46.1 & 8.371877670288084 & 0.00012260818 & -71.54612731933594 & 0.00020171217 & 0.008310039 & -0.0016196849 & 0.053329486 & 0.008098373 & 0.055937868 & 0.010129484 & 9.005262 & 7.461574 & 15.780102 & 0.00023697532 & 0.0012934689 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4690033750987052800 & 4690033750987052800 & 315031294 & 2016.0 & 8.371840808035467 & 0.018780315 & -71.54601783591016 & 0.017168758 & 1.175561329877746 & 0.019485082 & 60.33135 & 51.960773 & 49.55563900503472 & 0.024395725 & -15.6256432879165 & 0.022427745 & -0.11169319 & 0.15840806 & -0.46649227 & -0.013771435 & -0.2437631 & -0.023138085 & -0.06036153 & 0.025625324 & -0.15196364 & -0.15077655 & 347 & 0 & 346 & 1 & -0.29415616 & 344.88544 & 0.0 & 0.0 & 31 & false & 1.5212495 &  &  &  &  &  &  &  & 40 & 27 & 0.036059357 & 47 & 18 & 0 & 0.025526365 & 85.8961 & 0 & 0 & 0.9877837 & 0.12694792 & 0.075429924 & 0.045573 & 0.094468124 & 12.257596 & 49.46083 & -53.71573 & -38.785744 & false & 386 & 20062.75738619141 & 4.831002 & 4152.9185 & 14.931391 & 42 & 10043.877905178084 & 14.520534 & 691.7017 & 15.333789 & 42 & 14439.404933920876 & 14.56961 & 991.0633 & 14.349022 & 1.2203349 & 0 & 1 & 0 & 0 & 0 & 0.98476696 & 0.4023981 & 0.58236885 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 304.9573829449669 & -45.51157141103506 & 313.06778653208414 & -62.702367358239364 & false & false & 0 & true & true & false & false & false & true & true & false & 1.02546315e-13 & 5.1225636e-13 & 0.99994814 & 5090.223 & 5083.7466 & 5101.606 & 4.3357 & 4.3173 & 4.3481 & -1.3857 & -1.4113 & -1.3544 & 832.5712 & 817.1818 & 856.6956 & 0.0074 & 0.002 & 0.0168 & 0.006 & 0.0016 & 0.0137 & 0.0033 & 0.0009 & 0.0075 & MARCS & 0.43752909328171335 & 0.0 & 0.0 & 0.0 &  &  & 0.0 & 0 & 0.0 & 0.0 & 0 &  & 0.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0 \\
29124 & J004627-734621 & 00:46:27.07 & -73:46:20.9 & 11.61280059814453 & 0.00013693655 & -73.77247619628906 & 0.00023251561 & 0.006100434 & -0.0027022578 & 0.03693146 & 0.0058955266 & 0.0438542 & 0.008591367 & 9.945726 & 7.64292 & 5.618037 & 0.00017070891 & 0.0009686665 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4685776265879398656 & 4685776265879398656 & 1193746686 & 2016.0 & 11.61236180925975 & 1.3355746 & -73.77244339426248 & 1.2806226 & 1.494317178962959 & 1.3791072 & 1.0835395 & 10.906597 & -6.618982265937383 & 1.545366 & -8.66850205630162 & 2.7291965 & -0.015349186 & 0.14392607 & -0.32408223 & -0.18931045 & 0.25141767 & -0.22157729 & 0.20746915 & -0.096548 & -0.012520628 & -0.33320367 & 124 & 0 & 112 & 12 & 1.1328408 & 148.26959 & 3.7420943 & 1.5489331 & 95 & false &  & 1.083479 & 0.35800678 & -0.24171083 & -0.10616227 & -0.045399133 & 0.06214615 & 0.3349972 & 14 & 12 & 3.8795936 & 17 & 7 & 3 & 0.15762746 & 63.523464 & 6 & 0 & 1.0755806 & 0.27661675 & 0.0904547 & 0.26972005 & 0.07058556 & 101.7418 & 67.416824 & -50.373283 & -1.8558813 & false & 134 & 94.35341955189789 & 2.3622456 & 39.942257 & 20.750473 & 12 & 86.1422301605419 & 7.652205 & 11.257177 & 20.500502 & 11 & 115.77119168442631 & 8.745399 & 13.237953 & 19.588894 & 2.1399693 & 0 & 1 & 0 & 0 & 0 & 0.91160774 & -0.24997139 & 1.1615791 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 303.41116440080094 & -43.35116439427292 & 309.6482117777097 & -64.59587656667038 & false & false & 0 & false & false & false & false & false & false & false & false & 0.00011183102 & 8.595295e-06 & 0.9998766 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.4447278151564287 & 0.0 & 0.0 & 0.0 &  &  & 0.0 & 0 & 0.0 & 0.0 & 0 &  & 0.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0 \\
35036 & J004733-731701 & 00:47:33.22 & -73:17:01.0 & 11.888431549072264 & 0.0003120004 & -73.28359985351564 & 0.00043315152 & 0.015313439 & 0.010531575 & 0.09248572 & 0.012414323 & 0.4160283 & 0.101167165 & 16.970673 & 16.966326 & -2.098865 & -0.009028088 & 0.019170076 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4685942708820468224 & 4685942708820468224 & 252529496 & 2016.0 & 11.888189909583327 & 0.7313211 & -73.28354136925654 & 0.45674637 & 2.0876400317876325 & 0.53433347 & 3.9069984 & 12.808829 & -11.996496977056763 & 0.8054174 & -4.488893472352316 & 0.59961134 & 0.20010975 & -0.090462275 & -0.3875789 & 0.23767242 & 0.0065974947 & 0.1270276 & 0.32024974 & -0.08704879 & -0.10706768 & 0.08462222 & 193 & 0 & 176 & 17 & 9.057293 & 419.72995 & 3.5321283 & 16.640333 & 95 & false &  & 1.3319486 & 0.13550736 & 0.11685783 & 0.21874389 & 0.020464081 & 0.06112085 & 0.18870234 & 21 & 16 & 1.1672734 & 39 & 39 & 0 & 0.16606314 & 49.349846 & 0 & 84 & 1.5271927 & 0.12313676 & 0.46649402 & 0.17325388 & 0.09529518 & 71.43565 & -15.914573 & 56.93908 & -10.463708 & false & 198 & 301.54505529118825 & 3.6544027 & 82.51555 & 19.488987 & 0 &  &  &  &  & 0 &  &  &  &  &  &  &  &  &  & 0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 303.3192536163191 & -43.84178660900534 & 310.75477365952077 & -64.45927124165111 & false & false & 0 & false & false & false & false & false & false & false & false & 1.6938125e-06 & 0.0021403588 & 0.9978307 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.34375765832860106 & 0.0 & 0.0 & 0.0 &  &  & 0.0 & 0 & 0.0 & 0.0 & 0 &  & 0.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0 \\
49167 & J004752-732455 & 00:47:52.47 & -73:24:54.9 & 11.968629837036131 & 0.00013560058 & -73.41525268554688 & 0.00018431204 & 0.013071373 & -0.005924938 & 0.08144665 & 0.012872859 & 0.077086404 & 0.014307939 & 8.340066 & 7.2640185 & 2.2763748 & 0.00016890114 & 0.00082515186 & -2.77226 & 3.20614 &  &  & 3 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.024792524 & 11.968342 & -73.41512 & 0.12775044 & 0.024589138 & 0.131345 & 0.03250151 & 0.5528097777847764 &  &  &  &  &  &  &  &  & 0.026455885 & 11.96876 & -73.41538 & 0.18247627 & 0.026130386 & 0.18403877 & 0.03233265 & 0.48556686031564394 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4685926422305317504 & 4685926422305317504 & 941773337 & 2016.0 & 11.969079288461979 & 0.52705795 & -73.41534102206644 & 0.47229025 & 1.7048524655119206 & 0.5300319 & 3.216509 & 10.062103 & -8.753127309779982 & 0.67931134 & -4.962728894077333 & 0.6239764 & 0.038544636 & 0.145797 & -0.35653168 & -0.042297937 & -0.0763814 & -0.049159583 & 0.083444886 & -0.13515693 & -0.034588434 & -0.059805598 & 278 & 0 & 276 & 2 & 55.89063 & 4911.8506 & 5.1411076 & 124.83347 & 95 & false &  & 1.540872 & 0.13059364 & -0.13522208 & 0.07718209 & 0.06122393 & 0.12849873 & 0.16438031 & 32 & 24 & 0.97074866 & 38 & 38 & 0 & 0.09857569 & 70.39481 & 12 & 0 & 4.1986885 & 0.040600263 & 0.0478227 & 0.07708677 & 0.07945494 & -162.38719 & -20.809273 & -53.4951 & 20.682367 & false & 303 & 499.98176489653486 & 1.9708706 & 253.68573 & 18.939981 & 35 & 541.9813008028505 & 8.82239 & 61.432484 & 18.503582 & 34 & 329.1162547825413 & 7.112304 & 46.274208 & 18.454523 & 1.7422587 & 0 & 35 & 0 & 34 & 0 & 0.049058914 & -0.43639946 & 0.48545837 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 303.28350504361913 & -43.7104775450815 & 310.50107477872035 & -64.53658568768563 & false & false & 0 & false & false & false & false & false & false & false & false & 8.345449e-09 & 0.00020588917 & 0.9997866 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.5703357784630305 & 0.0 & 0.0 & 0.0 &  &  & 0.0 & 0 & 0.0 & 0.0 & 0 &  & 0.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0 \\
21946 & J005445-745554 & 00:54:45.49 & -74:55:53.9 & 13.689529418945307 & 0.000115212366 & -74.93164825439453 & 0.00016760464 & 0.007943802 & -0.0014559143 & 0.05919618 & 0.007594939 & 0.06559068 & 0.009664477 & 9.802645 & 7.2383614 & 18.95783 & 0.00018843617 & 0.0029179337 & 2.82182 & 3.46854 &  &  & 2 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.015449325 & 13.687661 & -74.93154 & 0.08976842 & 0.015381401 & 0.080762 & 0.01674553 & 1.7902743036203068 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4684753312040026112 & 4684753312040026112 & 746311393 & 2016.0 & 13.689852252133186 & 0.031734888 & -74.93155890926566 & 0.028821254 & 11.566194310638496 & 0.033914097 & 341.04385 & 38.763412 & 38.627360138334836 & 0.046279244 & -3.2448721076726628 & 0.037331067 & -0.07245673 & 0.096433125 & 0.092658654 & -0.01741157 & -0.104146205 & 0.030776301 & 0.22626573 & -0.19370593 & -0.2197111 & 0.024684157 & 350 & 0 & 349 & 1 & 1.296668 & 402.86505 & 0.13803226 & 1.8854734 & 31 & false & 1.2435392 &  &  &  &  &  &  &  & 40 & 27 & 0.064302534 & 48 & 16 & 0 & 0.010901798 & 86.94376 & 0 & 0 & 1.0488554 & 0.07550963 & 0.14049353 & 0.07755062 & 0.03566236 & -18.92745 & 17.367285 & 14.345207 & 27.231081 & false & 395 & 7444.484089984388 & 5.785659 & 1286.7133 & 16.00778 & 40 & 1104.4458761109397 & 7.1774654 & 153.87686 & 17.73068 & 41 & 9902.804695286684 & 19.999594 & 495.1503 & 14.7585 & 1.478578 & 0 & 0 & 0 & 0 & 0 & 2.9721804 & 1.7229004 & 1.24928 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 302.64054795246574 & -42.19481192767634 & 307.6288111590845 & -65.56198066652013 & false & false & 0 & true & false & false & false & false & true & true & false & 1.3750302e-13 & 6.88796e-13 & 0.99648726 & 3274.0312 & 3272.1897 & 3276.0486 & 4.9551 & 4.9528 & 4.9567 & -0.1148 & -0.1206 & -0.11 & 88.5686 & 88.3359 & 88.8117 & 0.8867 & 0.8763 & 0.8979 & 0.5553 & 0.5487 & 0.5625 & 0.3711 & 0.3669 & 0.3757 & MARCS & 0.4091389666865505 & 0.0 & 0.0 & 0.0 &  &  & 0.0 & 0 & 0.0 & 0.0 & 0 &  & 0.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0 \\
37152 & J005621-730647 & 00:56:20.66 & -73:06:46.6 & 14.086098670959474 & 0.00010302699 & -73.1129379272461 & 0.00011607202 & 0.0075130337 & 0.0063990327 & 0.06876776 & 0.0073481626 & 0.06720719 & 0.008334102 & 8.178067 & 7.6483107 & 2.7331 & -0.00016091789 & 0.0010359188 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4685912815770474368 & 4685912815770474368 & 293869927 & 2016.0 & 14.085700351931012 & 1.3979478 & -73.11303850828631 & 0.73954475 & 1.254243133796141 & 0.91950554 & 1.3640409 & 12.970659 & -12.091235310944363 & 1.6249541 & -4.694682215020553 & 0.94972116 & 0.14220664 & -0.27626678 & -0.7899619 & 0.0098526 & 0.2723021 & -0.12984632 & -0.23550753 & 0.23506545 & -0.30244198 & -0.0073003406 & 178 & 0 & 177 & 1 & 5.986517 & 329.40292 & 3.912607 & 5.4128704 & 95 & false &  & 0.568986 & 0.2706171 & -0.27113834 & -0.07381922 & 0.053713836 & 0.3110847 & -0.1501488 & 21 & 16 & 2.5416026 & 24 & 12 & 2 & 0.046486866 & 80.094055 & 0 & 4 & 1.3384478 & 0.22785333 & 0.27027774 & 0.1386494 & 0.1572233 & -2.332071 & -12.836806 & 4.9122953 & -3.177988 & false & 191 & 119.68953495303386 & 1.1290772 & 106.00651 & 20.492226 & 11 & 151.98949116364585 & 12.143073 & 12.516559 & 19.884008 & 11 & 108.56403105092487 & 12.754169 & 8.512042 & 19.65868 & 2.1769116 & 0 & 11 & 0 & 11 & 0 & 0.22532845 & -0.60821724 & 0.8335457 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 302.4366906160208 & -44.01049482781918 & 311.74209585207103 & -64.96390061295169 & false & false & 0 & false & false & false & false & false & false & false & false & 0.000685362 & 0.0035893936 & 0.99572515 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.5244727714599073 & 0.0 & 0.0 & 0.0 &  &  & 0.0 & 0 & 0.0 & 0.0 & 0 &  & 0.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0 \\
43267 & J005759-723741 & 00:57:59.21 & -72:37:40.8 & 14.496690750122077 & 0.0001476812 & -72.62799835205078 & 0.00020503448 & 0.011747763 & -0.004744904 & 0.07220545 & 0.0118118515 & 0.073828325 & 0.015077914 & 8.900792 & 7.3521605 & 0.12310777 & -1.8270318e-06 & 0.0010889713 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4685988613398832000 & 4685988613398832000 & 455607852 & 2016.0 & 14.49636953017558 & 0.77957857 & -72.62800901296376 & 0.78539747 & 2.5386107730113303 & 0.8157968 & 3.1118174 & 21.244772 & 21.145664238661123 & 1.2623805 & -2.0496927620499075 & 1.3171939 & 0.19817744 & 0.113674015 & 0.35345137 & 0.13308379 & -0.05935654 & 0.11584967 & 0.22382149 & -0.22840302 & -0.0375308 & 0.35278478 & 244 & 0 & 225 & 19 & 11.451896 & 590.193 & 5.411764 & 15.029851 & 95 & false &  & 2.1612058 & 0.20864727 & -0.24563044 & -0.084105335 & -0.034335766 & 0.06905214 & 0.020116713 & 29 & 22 & 2.0987437 & 38 & 27 & 2 & 0.40777123 & 113.76453 & 59 & 21 & 1.5926366 & 0.05749847 & 0.11043585 & 0.13188331 & 0.1159102 & -162.92752 & -40.49021 & 22.52154 & 15.626724 & false & 264 & 164.52334363913064 & 3.5772753 & 45.991245 & 20.146797 & 0 &  &  &  &  & 0 &  &  &  &  &  &  &  &  &  & 1 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 302.2468768955441 & -44.491530940780045 & 312.9012418132682 & -64.87206123641546 & false & false & 0 & false & false & false & false & false & false & false & false & 6.8006325e-09 & 2.859807e-10 & 0.99997944 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.36561116785152503 & 0.0 & 0.0 & 0.0 &  &  & 0.0 & 0 & 0.0 & 0.0 & 0 &  & 0.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0 \\
16681 & J005815-744629 & 00:58:14.85 & -74:46:29.0 & 14.561874389648438 & 0.00013442498 & -74.77471923828125 & 0.00015436843 & 0.008990852 & 0.0010280097 & 0.063517965 & 0.008876061 & 0.061479785 & 0.009956975 & 8.309153 & 7.458785 & 24.42395 & 1.1758199e-05 & 0.0021699031 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4684760561944723456 & 4684760561944723456 & 1193820043 & 2016.0 & 14.562220517090937 & 0.02393001 & -74.77460533134116 & 0.022610772 & 1.136337587463208 & 0.026024839 & 43.663578 & 29.383705 & 29.248647115373434 & 0.03564541 & -2.8140363788578027 & 0.030269587 & -0.0448546 & 0.18546276 & 0.020283137 & 0.02039883 & -0.04279942 & 0.06253483 & 0.19573677 & -0.11245558 & -0.12280608 & 0.022605214 & 344 & 0 & 342 & 2 & -2.3119047 & 292.0102 & 0.0 & 0.0 & 31 & false & 1.4844615 &  &  &  &  &  &  &  & 40 & 25 & 0.04938854 & 45 & 12 & 0 & 0.009677182 & 51.85982 & 0 & 0 & 0.9113247 & 0.09134744 & 0.10748413 & 0.06941962 & 0.15446456 & -6.1152883 & 15.0607 & 1.0092767 & 26.353271 & false & 382 & 10686.196597221082 & 3.1740272 & 3366.7627 & 15.615309 & 41 & 4951.526448894958 & 15.66961 & 315.9955 & 16.101694 & 40 & 8159.623335969001 & 11.170606 & 730.4549 & 14.96872 & 1.2269238 & 0 & 1 & 0 & 0 & 0 & 1.1329737 & 0.48638535 & 0.6465883 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 302.3269760610514 & -42.34564362388885 & 308.1803509119716 & -65.71959500701713 & false & false & 0 & true & false & false & false & false & true & true & false & 1.02855556e-13 & 5.1379425e-13 & 0.99991757 & 4904.219 & 4882.476 & 4924.6265 & 4.514 & 4.4967 & 4.5284 & 0.0677 & 0.0426 & 0.0943 & 871.0646 & 849.9078 & 896.2961 & 0.0739 & 0.0551 & 0.0915 & 0.0585 & 0.0435 & 0.0726 & 0.0308 & 0.0229 & 0.0382 & MARCS & 0.5327137978778305 & 0.0 & 0.0 & 0.0 &  &  & 0.0 & 0 & 0.0 & 0.0 & 0 &  & 0.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0 \\
33424 & J010338-732726 & 01:03:38.34 & -73:27:25.8 & 15.909752845764158 & 0.00038931196 & -73.45716094970702 & 0.00032873635 & 0.008329975 & 0.0063669826 & 0.046227857 & 0.007547987 & 0.10306968 & 0.02694533 & 12.714072 & 11.22382 & -6.7658625 & -0.0034951211 & 0.00662466 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4685691573434514176 & 4685691573434514176 & 174509790 & 2016.0 & 15.90942276653968 & 0.5558217 & -73.45729098831696 & 0.6465893 & -1.0724367334071518 & 0.6107631 & -1.7558966 & 10.246624 & -5.597533294620236 & 0.8724506 & 8.5825937359585 & 0.8962911 & -0.019638196 & 0.1418671 & -0.02389202 & -0.039967723 & -0.09799591 & 0.04036124 & 0.55439293 & -0.1309265 & -0.15438919 & 0.09632541 & 257 & 0 & 256 & 1 & 47.162163 & 3840.6604 & 5.716023 & 120.472176 & 95 & false &  & 1.279919 & 0.1518248 & 0.015397215 & -0.0014661014 & 0.068240814 & -0.0077987085 & -0.1908832 & 30 & 22 & 1.3294574 & 37 & 10 & 4 & 0.111359246 & 159.59276 & 56 & 8 & 3.7301896 & 0.12091118 & 0.041810896 & 0.25742406 & 0.08057469 & 47.88069 & -4.9976053 & 53.110264 & -43.207596 & false & 250 & 558.6608626628421 & 3.370814 & 165.7347 & 18.819496 & 29 & 618.1340779770908 & 10.784663 & 57.31603 & 18.360836 & 30 & 663.428201588075 & 7.4971895 & 88.49026 & 17.69341 & 2.2939897 & 0 & 29 & 0 & 30 & 0 & 0.66742516 & -0.45866013 & 1.1260853 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 301.73237349026783 & -43.64253312878524 & 311.4814808093448 & -65.58171682194298 & false & false & 0 & false & false & false & false & false & false & false & false & 3.6180148e-07 & 0.005135199 & 0.99485254 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.5593011850533312 & 0.0 & 0.0 & 0.0 &  &  & 0.0 & 0 & 0.0 & 0.0 & 0 &  & 0.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0 \\
50096 & J010631-714838 & 01:06:31.12 & -71:48:38.5 & 16.62967491149903 & 0.00018127287 & -71.8106918334961 & 0.00020585778 & 0.008278559 & -0.004990244 & 0.05176147 & 0.00779529 & 0.07245652 & 0.013272099 & 10.057983 & 8.909426 & 14.566725 & -0.00049559365 & 0.0027533474 & -2.59258 & 0.917326 &  &  & 2 &  &  &  &  &  &  &  &  &  &  & 0.038986843 & 16.63048 & -71.81086 & 0.21834922 & 0.038921677 & 0.15690832 & 0.031574223 & 1.0877812122168597 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4690540282257021440 & 4690540282257021440 & 942884357 & 2016.0 & 16.629275636068712 & 0.85869795 & -71.81068074610548 & 0.7122809 & 0.20608157030493868 & 0.81069815 & 0.2542026 & 10.929194 & 4.658713481329512 & 1.6756259 & -9.886540288421912 & 2.1032624 & -0.18300006 & -0.22932845 & -0.42471185 & -0.11967068 & 0.3201851 & -0.18762892 & 0.32483703 & 0.32939562 & -0.16344862 & -0.5033541 & 163 & 0 & 163 & 0 & 0.7473508 & 177.2645 & 0.0 & 0.0 & 95 & false &  & 1.6590705 & 0.21218038 & -0.1950347 & 0.16650377 & 0.08642985 & -0.065038964 & 0.16075033 & 19 & 14 & 3.2712412 & 23 & 6 & 0 & 0.0971569 & 128.81276 & 0 & 0 & 1.0403185 & 0.0068341563 & 0.28324223 & 0.16661277 & 0.23944314 & -38.882263 & 32.144043 & 42.726715 & -21.527838 & false & 184 & 109.88141829007648 & 1.2415806 & 88.501236 & 20.585056 & 20 & 82.88715450041423 & 6.074722 & 13.644601 & 20.542324 & 20 & 90.07474872951343 & 8.797104 & 10.239137 & 19.861387 & 1.5740778 & 0 & 0 & 0 & 0 & 0 & 0.6809368 & -0.04273224 & 0.72366905 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 301.26082622907563 & -45.268610233034124 & 315.3045884624995 & -65.11719262932931 & false & false & 0 & false & false & false & false & false & false & false & false & 5.2272546e-05 & 9.406854e-07 & 0.9999287 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.44218601300469335 & 0.0 & 0.0 & 0.0 &  &  & 0.0 & 0 & 0.0 & 0.0 & 0 &  & 0.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0 \\
103644 & J010711-753224 & 01:07:11.07 & -75:32:24.1 & 16.796131134033203 & 5.1646737e-05 & -75.54002380371094 & 4.8089732e-05 & 0.009902897 & -0.00027944756 & 0.20758617 & 0.009587693 & 0.2281315 & 0.012163416 & 8.425386 & 8.356398 & 89.171455 & 0.00033966466 & 0.0032004963 & -0.852105 & 0.359528 & 2.9122 & 0.362128 & 10 & 0.041279748 & 01:07:11.04 & -75:32:23.6 & 16.795982 & -75.53988 & 0.35710648 & 0.04024455 & 0.37978458 & 0.050098456 & 0.5387149852103155 &  &  &  &  &  &  &  &  & 0.034125436 & 16.796797 & -75.54004 & 0.30247352 & 0.03219236 & 0.37960982 & 0.04753862 & 0.600903773046843 & 0.029745746 & 16.796324 & -75.53982 & 0.2630603 & 0.028507013 & 0.30611092 & 0.039442968 & 0.7615285865194232 & 0.029972373 & 16.796595 & -75.53998 & 0.21665439 & 0.029192822 & 0.22417533 & 0.03522198 & 0.4480502367979536 &  &  &  &  &  &  &  &  & 0.025842106 & 16.796165 & -75.539894 & 0.18249664 & 0.025297927 & 0.18232557 & 0.029570773 & 0.4679378151005506 & 0.02103743 & 16.795528 & -75.53994 & 0.18542184 & 0.019580785 & 0.24446604 & 0.02963071 & 0.6203509769422885 & 0.019352805 & 16.79606 & -75.540115 & 0.17211904 & 0.01884391 & 0.17710295 & 0.022586616 & 0.3356396876890986 & 0.025973681 & 16.795841 & -75.53998 & 0.20230974 & 0.024677118 & 0.25923616 & 0.037750565 & 0.3083476447437536 &  &  &  &  &  &  &  &  & 0.03458255 & 16.79615 & -75.54034 & 0.24106136 & 0.033552438 & 0.25909778 & 0.04255247 & 1.1262291519596608 & 1636148068921376768 & Gaia DR3 4684485198699244672 & 4684485198699244672 & 1435209586 & 2016.0 & 16.796470508599405 & 0.14742972 & -75.54004417322268 & 0.12795825 & 6.201811955836491 & 0.15825228 & 39.1894 & 30.066357 & 27.16930309923411 & 0.21990867 & 12.876908573030768 & 0.17208187 & -0.11506013 & -0.0319526 & -0.13984531 & 0.08031358 & -0.18119562 & 0.12740435 & 0.019365923 & -0.12368352 & -0.31217036 & 0.0649405 & 325 & 0 & 325 & 0 & -0.06588709 & 386.99036 & 0.5573575 & 1.5256587 & 95 & false &  & 1.1777729 & 0.04054372 & -0.069675684 & 0.099961475 & -0.24765722 & 0.079350784 & 0.14018697 & 37 & 26 & 0.30679035 & 45 & 16 & 0 & 0.022949578 & 87.988716 & 0 & 0 & 0.9963488 & 0.050591473 & 0.11819837 & 0.08416022 & 0.120384336 & 78.05882 & 10.7833395 & 18.940529 & 36.9201 & false & 351 & 672.4202112285665 & 1.4221247 & 472.82785 & 18.618265 & 36 & 148.7184887827393 & 6.741732 & 22.05939 & 19.907629 & 41 & 1105.3429526503098 & 8.899319 & 124.205345 & 17.139153 & 1.8649967 & 0 & 0 & 0 & 0 & 0 & 2.7684765 & 1.2893639 & 1.4791126 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 301.6192633217558 & -41.54804386043586 & 306.8492479417771 & -66.50877070116799 & false & false & 0 & false & false & false & false & false & false & false & false & 4.8918616e-11 & 2.0851745e-09 & 0.9998808 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.3161474837512843 & 0.0 & 0.0 & 0.0 &  &  & 0.0 & 0 & 0.0 & 0.0 & 0 &  & 0.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0 \\
98866 & J010746-704641 & 01:07:45.88 & -70:46:41.0 & 16.941146850585934 & 5.123522e-05 & -70.77804565429688 & 5.2911655e-05 & 0.009746948 & -0.0008036513 & 0.19274853 & 0.009373091 & 0.20730498 & 0.011629105 & 8.616414 & 7.995086 & -6.586397 & -0.00016429691 & 0.002550688 & -0.174988 & 0.32977 & 1.15389 & -0.338886 & 8 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.026989428 & 16.94159 & -70.77812 & 0.16869646 & 0.02525491 & 0.25190985 & 0.04688301 & 0.5920316407962767 & 0.025541317 & 16.941376 & -70.77807 & 0.18869887 & 0.024552863 & 0.21667862 & 0.03309106 & 0.2835134523754089 & 0.025881339 & 16.941069 & -70.77814 & 0.18064472 & 0.025399312 & 0.18400888 & 0.030929241 & 0.34237422296740266 &  &  &  &  &  &  &  &  & 0.023645487 & 16.94125 & -70.778175 & 0.24161415 & 0.023152767 & 0.22309634 & 0.024387484 & 0.48261299752267955 & 0.02001918 & 16.940866 & -70.77802 & 0.21287183 & 0.019552685 & 0.20991224 & 0.022313993 & 0.342376098554244 & 0.01980171 & 16.941319 & -70.77791 & 0.17166826 & 0.019307178 & 0.16960469 & 0.022146273 & 0.5346132293975121 & 0.02706154 & 16.940838 & -70.77839 & 0.22018579 & 0.026026703 & 0.24103418 & 0.032947212 & 1.2890765895720406 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4690832683625105152 & 4690832683625105152 & 648266382 & 2016.0 & 16.941367281349798 & 0.7834192 & -70.77808598674464 & 0.6136636 & 1.0254853988777828 & 0.7337753 & 1.3975469 & 12.377615 & 12.123676470745648 & 1.2649093 & 2.4943559156588675 & 0.94090116 & -0.07300006 & 0.11105722 & 0.31095088 & -0.07205228 & 0.043075826 & -0.06321405 & 0.33541903 & -0.21123093 & -0.04167686 & 0.15275067 & 256 & 0 & 252 & 4 & 6.264286 & 434.3875 & 4.088004 & 7.41661 & 95 & false &  & 1.5879599 & 0.21520121 & -0.10400936 & 0.1459592 & -0.13453908 & 0.100964926 & 0.11498452 & 29 & 21 & 1.7920929 & 33 & 7 & 1 & 0.050331518 & 35.96636 & 9 & 3 & 1.293842 & 0.11793971 & 0.22922616 & 0.0038666953 & 0.08422593 & -20.548996 & 1.8527037 & -6.9723244 & -7.1211143 & false & 277 & 130.9299607138572 & 0.9986124 & 131.1119 & 20.39477 & 24 & 49.85576243572282 & 5.320305 & 9.370847 & 21.094254 & 27 & 245.045134729438 & 10.480724 & 23.380554 & 18.77478 & 2.252356 & 0 & 24 & 0 & 27 & 0 & 2.3194733 & 0.6994839 & 1.6199894 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 300.98844900280085 & -46.288502284478646 & 317.59974466202766 & -64.75516759974171 & false & false & 0 & false & false & false & false & false & false & false & false & 3.6533336e-09 & 3.1566613e-06 & 0.99997395 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.26179683166795337 & 0.0 & 0.0 & 0.0 &  &  & 0.0 & 0 & 0.0 & 0.0 & 0 &  & 0.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0 \\
75076 & J011249-701317 & 01:12:48.53 & -70:13:17.0 & 18.202198028564453 & 0.00011256346 & -70.22139739990234 & 9.010505e-05 & 0.009938986 & 0.0001706623 & 0.10131365 & 0.009616505 & 0.10933139 & 0.012059289 & 8.690444 & 7.9578085 & 81.56846 & 0.0011728584 & 0.0040501375 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4690956138162512256 & 4690956138162512256 & 1788925145 & 2016.0 & 18.201999140613538 & 0.04735883 & -70.2214446096651 & 0.036044605 & 0.3234962893267796 & 0.043771528 & 7.3905644 & 20.541145 & -2.6506865805578084 & 0.06207127 & -20.36940082638725 & 0.04731518 & -0.019226532 & -0.057150695 & -0.53400654 & 0.055111118 & -0.019004082 & -0.0041475985 & -0.10364747 & 0.14323133 & -0.30921724 & -0.14785725 & 363 & 0 & 363 & 0 & 0.3398476 & 381.63226 & 0.0 & 0.0 & 31 & false & 1.5925624 &  &  &  &  &  &  &  & 42 & 27 & 0.091444306 & 47 & 19 & 0 & 0.01815597 & 85.614044 & 0 & 0 & 1.0117927 & 0.0864329 & 0.119525574 & 0.024199158 & 0.08838427 & 29.866062 & 10.628787 & 56.646862 & 12.091154 & false & 387 & 3827.819913040797 & 2.2919216 & 1670.1356 & 16.729988 & 43 & 2217.6271397366095 & 9.129692 & 242.90273 & 16.973822 & 44 & 2449.5720463901325 & 8.565415 & 285.98404 & 16.27517 & 1.2192839 & 0 & 23 & 0 & 21 & 0 & 0.69865227 & 0.24383354 & 0.45481873 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 300.2940334265431 & -46.79719847270629 & 319.2141667542979 & -64.87761191873885 & false & false & 0 & true & false & false & false & false & true & true & false & 2.3193833e-10 & 2.0028434e-12 & 0.9999596 & 6346.337 & 6288.7344 & 6378.394 & 4.4311 & 4.3866 & 4.4584 & -2.7566 & -3.2052 & -2.4789 & 2563.5376 & 2464.9697 & 2752.521 & 0.1597 & 0.1311 & 0.1758 & 0.1383 & 0.1134 & 0.1524 & 0.0761 & 0.0624 & 0.0839 & MARCS & 0.32431456590311414 & 0.0 & 0.0 & 0.0 &  &  & 0.0 & 0 & 0.0 & 0.0 & 0 &  & 0.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0 \\
54927 & J012221-714122 & 01:22:20.77 & -71:41:22.2 & 20.586557388305664 & 0.00020361457 & -71.68950653076172 & 0.00020525897 & 0.009052881 & -0.0010124868 & 0.053160314 & 0.008673951 & 0.07249566 & 0.0147304265 & 9.895717 & 8.825937 & 16.446533 & -0.00042885047 & 0.00279627 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4687587337618874240 & 4687587337618874240 & 1538668752 & 2016.0 & 20.586470576263487 & 0.1749816 & -71.68941275626388 & 0.1758489 & 0.20642576097858487 & 0.19623473 & 1.0519328 & 18.381905 & -2.3768476327307457 & 0.22328687 & -18.22758896198867 & 0.21109295 & -0.07324629 & 0.14631501 & -0.109368786 & -0.06865289 & -0.27175808 & 0.02102075 & 0.15736374 & -0.11003814 & -0.24042137 & 0.04157719 & 345 & 0 & 344 & 1 & 0.044852097 & 351.95996 & 0.0 & 0.0 & 95 & false &  & 1.4677447 & 0.049638156 & -0.07672238 & 0.20405889 & -0.15629734 & 0.1292548 & 0.00088407524 & 39 & 28 & 0.31363472 & 45 & 45 & 0 & 0.03475402 & 82.80692 & 0 & 17 & 1.000739 & 0.06476936 & 0.046584696 & 0.07720641 & 0.092319615 & 136.89204 & 10.979014 & 27.743921 & 20.769144 & false & 377 & 415.10180557654047 & 0.944415 & 439.53326 & 19.141981 & 0 &  &  &  &  & 0 &  &  &  &  &  &  &  &  &  & 0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 299.49320954818796 & -45.23190506390177 & 316.7896192710313 & -66.20136572372756 & false & false & 0 & false & false & false & false & false & false & false & false & 1.1788849e-07 & 1.4483618e-06 & 0.9999774 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.3242057172367397 & 0.0 & 0.0 & 0.0 &  &  & 0.0 & 0 & 0.0 & 0.0 & 0 &  & 0.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0 \\
27921 & J012740-734651 & 01:27:39.77 & -73:46:50.6 & 21.915710449218746 & 0.00017020793 & -73.78073120117188 & 0.000113031696 & 0.008942525 & -0.0026908289 & 0.06778494 & 0.008516196 & 0.082718015 & 0.012484188 & 9.440816 & 8.278199 & 83.54534 & -0.00011372381 & 0.0012429453 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4686223290360321664 & 4686223290360321664 & 155364710 & 2016.0 & 21.91561367119415 & 1.5531114 & -73.78075760204426 & 1.364934 & 4.808589343177136 & 1.5345356 & 3.1335795 & 36.179962 & 30.645147072299768 & 2.8355236 & 19.231868208193745 & 2.2337563 & -0.28029376 & -0.065677956 & 0.49208426 & 0.05981465 & 0.27062157 & 0.03495764 & 0.010263563 & -0.29563242 & -0.24470948 & -0.1180108 & 110 & 0 & 109 & 1 & 2.1487224 & 140.13615 & 0.0 & 0.0 & 95 & false &  & 0.27898178 & 0.43263397 & -0.13000977 & 0.29745454 & -0.3124912 & 0.31964657 & 0.07070507 & 13 & 12 & 4.044425 & 16 & 4 & 0 & 0.09598549 & 159.68253 & 1 & 0 & 1.1499919 & 0.30384672 & 0.25052467 & 0.19433966 & 0.26744023 & -35.84604 & 43.649124 & 9.991526 & 25.749275 & false & 132 & 84.81767576322997 & 1.16691 & 72.6857 & 20.866152 & 6 & 30.2562371630513 & 7.078781 & 4.2742157 & 21.636505 & 15 & 129.92526225507305 & 7.8597674 & 16.53042 & 19.463661 & 1.8885391 & 0 & 0 & 0 & 0 & 0 & 2.172844 & 0.7703533 & 1.4024906 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 299.47972196319904 & -43.10383522841777 & 312.14842488222763 & -67.28470387725649 & false & false & 0 & false & false & false & false & false & false & false & false & 4.416789e-08 & 6.0188204e-06 & 0.99998665 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.15900549369326736 & 0.0 & 0.0 & 0.0 &  &  & 0.0 & 0 & 0.0 & 0.0 & 0 &  & 0.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0 \\
37203 & J013527-725507 & 01:35:27.13 & -72:55:07.5 & 23.863046646118164 & 0.00014658898 & -72.91873931884766 & 8.703462e-05 & 0.011865184 & -0.002072677 & 0.09850891 & 0.011603055 & 0.09436492 & 0.013033629 & 8.433087 & 7.277375 & 83.18401 & 0.0001791455 & 0.0023451408 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4686843586718702464 & 4686843586718702464 & 712824348 & 2016.0 & 23.863295574270058 & 0.45437878 & -72.91880297890562 & 0.38014102 & 2.949602216190911 & 0.45440933 & 6.491069 & 24.417515 & -20.90595498016153 & 0.5012416 & -12.615706934135163 & 0.5196264 & -0.08529176 & 0.29903257 & -0.18422154 & -0.19543116 & 0.072975144 & -0.08443873 & -0.24198839 & -0.092235714 & -0.29169223 & -0.04868715 & 319 & 0 & 315 & 4 & 1.2843539 & 383.9847 & 1.1479739 & 0.81630987 & 95 & false &  & 1.1267123 & 0.13201264 & -0.15856895 & 0.1284599 & -0.040724862 & 0.027538877 & 0.16172865 & 37 & 24 & 0.74233896 & 47 & 47 & 0 & 0.010032344 & 24.902006 & 0 & 0 & 1.0510097 & 0.22437298 & 0.12915088 & 0.062190194 & 0.0680404 & 24.010094 & 31.137897 & 30.896896 & -20.230991 & false & 372 & 163.3299585894174 & 0.7853622 & 207.9677 & 20.154703 & 35 & 30.005536255483516 & 3.5980628 & 8.339358 & 21.645538 & 41 & 255.7568903979835 & 7.540648 & 33.9171 & 18.728327 & 1.7496021 & 0 & 0 & 0 & 0 & 0 & 2.9172115 & 1.4908352 & 1.4263763 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 298.47482856619365 & -43.82651244322956 & 314.7250464284086 & -67.55986944810252 & false & false & 0 & false & false & false & false & false & false & false & false & 2.2328339e-11 & 5.156427e-13 & 0.99999267 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.3293335459106622 & 0.0 & 0.0 & 0.0 &  &  & 0.0 & 0 & 0.0 & 0.0 & 0 &  & 0.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0 \\
69849 & J014028-702341 & 01:40:27.60 & -70:23:41.0 & 25.115016937255863 & 0.0003464727 & -70.39472198486328 & 0.0004004187 & 0.02351523 & -0.0015891204 & 0.1290607 & 0.019783104 & 0.3962387 & 0.08879016 & 16.26853 & 12.109007 & 17.776022 & -0.0059833527 & 0.02236765 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 1636148068921376768 & Gaia DR3 4688123860632580352 & 4688123860632580352 & 941017819 & 2016.0 & 25.11519540288319 & 0.18721937 & -70.3946345475874 & 0.17266464 & 0.5398904212059916 & 0.19540948 & 2.762867 & 10.098518 & 10.089365060255474 & 0.24055794 & 0.4298666074944574 & 0.23797736 & 0.0019697656 & 0.18212594 & -0.43232659 & -0.1657651 & 0.18262497 & -0.041910253 & 0.02823036 & 0.048632126 & -0.27499235 & 0.06775567 & 317 & 0 & 314 & 3 & 0.2657448 & 337.92316 & 0.0 & 0.0 & 95 & false &  & 1.3101894 & 0.05433042 & 0.017503923 & 0.033790547 & -0.039760623 & 0.05553995 & -0.09179587 & 37 & 27 & 0.3545822 & 42 & 17 & 0 & 0.01773434 & 95.45041 & 0 & 0 & 1.0096403 & 0.07026646 & 0.1053236 & 0.042048566 & 0.03251257 & 42.81236 & 41.166626 & -50.20981 & 26.072863 & false & 341 & 429.3193059977312 & 1.074301 & 399.62668 & 19.105415 & 14 & 110.63871442894845 & 9.39623 & 11.774798 & 20.228775 & 14 & 496.6552717825752 & 25.453573 & 19.512203 & 18.007757 & 1.4145509 & 0 & 0 & 0 & 1 & 0 & 2.2210178 & 1.1233597 & 1.0976582 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & NOT_AVAILABLE & 297.0287823146951 & -46.16764734541863 & 321.2255578200852 & -67.06419289928353 & false & false & 0 & false & false & false & false & false & false & false & false & 1.1482838e-13 & 5.4127617e-13 & 0.99987376 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.3941243810118586 & 0.0 & 0.0 & 0.0 &  &  & 0.0 & 0 & 0.0 & 0.0 & 0 &  & 0.0 &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & 0.0 \\
\hline
  \end{tabular}
 \end{center}
\end{table*}

==> tables/silver_sample2.tex <==
\begin{table}
\begin{tabular}{cccccccc}
mainID & Name & RA2000 & DEC2000 & designation & pm & $p_\mathrm{star}$ & main\_type \\
81880  &  J002127-724852  &  00:21:27.23  &  -72:48:52.0  &  Gaia DR3 4689524951978390528  & 1.52 & - &  RRLyr  \\ 
47566  &  J002349-720538  &  00:23:49.25  &  -72:05:37.7  &  Gaia DR3 4689637995534546560  & 6.46 & 0.9996 &  X  \\ 
41486  &  J002927-723724  &  00:29:26.96  &  -72:37:24.1  &  Gaia DR3 4688791985744662016  & 1.38 & 0.999997 &  RGB*\_Candidate  \\ 
97311  &  J003320-732644  &  00:33:19.66  &  -73:26:44.0  &  Gaia DR3 4688834115109717632  & 1.21 & 0.99999 &  RGB*\_Candidate  \\ 
27187  &  J003525-712907  &  00:35:24.77  &  -71:29:07.3  &  Gaia DR3 4690023954169495296  & 1.62 & 0.99999 &  RGB*\_Candidate  \\ 
46634  &  J003550-720815  &  00:35:50.43  &  -72:08:14.8  &  Gaia DR3 4689195437801437568  & 3.31 & 0.9997 &  Star  \\ 
2940  &  J004050-733227  &  00:40:50.18  &  -73:32:26.7  &  Gaia DR3 4685841691137302144  & 1.2 & 0.999992 &  Star  \\ 
108082  &  J004136-730900  &  00:41:35.84  &  -73:08:59.5  &  Gaia DR3 4688866275834545536  & 1.47 & 0.999991 &  RGB*\_Candidate  \\ 
63250  &  J004231-741155  &  00:42:31.07  &  -74:11:55.0  &  Gaia DR3 4685749263432487040  & 5.96 & 0.99993 &  Star  \\ 
68845  &  J004236-704241  &  00:42:36.31  &  -70:42:40.8  &  Gaia DR3 4690363432675526528  & 1.23 & 0.999991 &  RGB*\_Candidate  \\ 
104480  &  J004313-725959  &  00:43:12.94  &  -72:59:58.6  &  Gaia DR3 4688876343239370240  & - & - &  YSO  \\ 
102448  &  J004403-743734  &  00:44:03.49  &  -74:37:34.0  &  Gaia DR3 4685490259707560832  & 31.4 & 0.9998 &  RotV*  \\ 
27171  &  J004413-735524  &  00:44:13.05  &  -73:55:23.8  &  Gaia DR3 4685757642897920256  & 1.32 & 0.999992 &  RGB*\_Candidate  \\ 
951  &  J004452-725734  &  00:44:51.97  &  -72:57:33.6  &  Gaia DR3 4688875140650831232  & - & - &  YSO\_Candidate  \\ 
40438  &  J004501-724905  &  00:45:00.97  &  -72:49:04.7  &  Gaia DR3 4688879951011299840  & 1.32 & 0.99997 &  Star  \\ 
7129  &  J004555-732410  &  00:45:55.10  &  -73:24:10.1  &  Gaia DR3 4685836331015987712  & 0.795 & 0.0 &  YSO\_Candidate  \\ 
35549  &  J004618-731243  &  00:46:17.68  &  -73:12:43.2  &  Gaia DR3 4685854129363535744  & 1.7 & 0.999994 &  Star  \\ 
6340  &  J004625-735051  &  00:46:25.41  &  -73:50:50.7  &  Gaia DR3 4685763247846544256  & 1.31 & 0.999992 &  RGB*\_Candidate  \\ 
1892  &  J004801-731328  &  00:48:01.41  &  -73:13:28.5  &  Gaia DR3 4685943911397856128  & - & - &  YSO\_Candidate  \\ 
64635  &  J004830-710415  &  00:48:30.35  &  -71:04:14.5  &  Gaia DR3 4690106417535980544  & 1.65 & 0.0 &  RRLyr  \\ 
96711  &  J004842-732615  &  00:48:41.85  &  -73:26:15.3  &  Gaia DR3 4685925288414794368  & 1.63 & 0.9994 &  YSO  \\ 
105644  &  J004845-731024  &  00:48:44.97  &  -73:10:24.3  &  Gaia DR3 4685944495526587776  & 7.08 & 0.994 &  RGB*\_Candidate  \\ 
86523  &  J004853-732458  &  00:48:53.45  &  -73:24:57.5  &  Gaia DR3 4685925868209190528  & - & 0.0 &  YSO\_Candidate  \\ 
187  &  J004903-733654  &  00:49:02.84  &  -73:36:54.0  &  Gaia DR3 4685872683646333952  & 1.2 & 0.999999 &  RGB*\_Candidate  \\ 
46787  &  J005105-722059  &  00:51:04.77  &  -72:20:58.9  &  Gaia DR3 4689036803221299840  & 1.31 & 0.999993 &  Star  \\ 
34243  &  J005143-732210  &  00:51:43.47  &  -73:22:09.7  &  Gaia DR3 4685885740348760576  & 1.59 & 0.999999 &  RGB*\_Candidate  \\ 
57423  &  J005205-744649  &  00:52:04.85  &  -74:46:49.3  &  Gaia DR3 4684816740118487936  & 32.8 & 0.999 &  Star  \\ 
48593  &  J005226-721247  &  00:52:26.32  &  -72:12:47.0  &  Gaia DR3 4689062057631896960  & 1.38 & 0.999995 &  RGB*\_Candidate  \\ 
106904  &  J005251-733203  &  00:52:51.36  &  -73:32:03.0  &  Gaia DR3 4685868075174097792  & - & 0.0 &  YSO\_Candidate  \\ 
775  &  J005307-732214  &  00:53:07.34  &  -73:22:14.1  &  Gaia DR3 4685882854092855808  & - & - &  RGB*\_Candidate  \\ 
100890  &  J005311-732800  &  00:53:10.56  &  -73:28:00.4  &  Gaia DR3 4685869625627356416  & 1.35 & 0.999995 &  Star  \\ 
97185  &  J005325-710243  &  00:53:25.46  &  -71:02:42.7  &  Gaia DR3 4689370676764568576  & 37.4 & 0.9998 &  Star  \\ 
33399  &  J005330-732720  &  00:53:30.40  &  -73:27:20.1  &  Gaia DR3 4685869655651182976  & 1.48 & 0.99999 &  RGB*\_Candidate  \\ 
31370  &  J005333-733708  &  00:53:33.38  &  -73:37:07.8  &  Gaia DR3 4685864024949338496  & 0.703 & - &  RRLyr  \\ 
107463  &  J005405-723802  &  00:54:04.87  &  -72:38:01.6  &  Gaia DR3 4688987703111747200  & 4.31 & - &  RRLyr  \\ 
36840  &  J005457-730813  &  00:54:56.53  &  -73:08:13.4  &  Gaia DR3 4685913228143892480  & 1.12 & 0.999995 &  RGB*\_Candidate  \\ 
95047  &  J005607-724723  &  00:56:06.53  &  -72:47:23.3  &  Gaia DR3 4685980401448794880  & 1.74 & 0.6 &  YSO  \\ 
2371  &  J005611-724749  &  00:56:10.82  &  -72:47:49.2  &  Gaia DR3 4685980435808569344  & 5.89 & 0.0 &  Star  \\ 
95001  &  J005806-720408  &  00:58:06.42  &  -72:04:07.7  &  Gaia DR3 4689021066425683328  & 4.87 & - &  YSO\_Candidate  \\ 
46590  &  J005854-722231  &  00:58:53.61  &  -72:22:30.5  &  Gaia DR3 4688998423409163136  & 1.38 & 0.999999 &  Star  \\ 
105021  &  J005951-721635  &  00:59:50.58  &  -72:16:35.1  &  Gaia DR3 4690503409984835328  & - & 0.96 &  YSO  \\ 
39379  &  J010027-725610  &  01:00:26.99  &  -72:56:10.3  &  Gaia DR3 4685919859574818944  & 1.65 & 0.99999 &  RGB*\_Candidate  \\ 
103281  &  J010150-743116  &  01:01:50.02  &  -74:31:15.6  &  Gaia DR3 4684789595926464000  & - & - &  RGB*\_Candidate  \\ 
49756  &  J010246-721240  &  01:02:46.23  &  -72:12:40.2  &  Gaia DR3 4690501902445562112  & - & 0.0 &  YSO\_Candidate  \\ 
16  &  J010308-714953  &  01:03:07.85  &  -71:49:52.6  &  Gaia DR3 4690530661527470976  & - & 0.0 &  YSO\_Candidate  \\ 
33010  &  J010314-705059  &  01:03:14.46  &  -70:50:59.0  &  Gaia DR3 4690839693019667840  & 6.83 & - &  Star  \\ 
48036  &  J010330-721550  &  01:03:30.41  &  -72:15:49.6  &  Gaia DR3 4687504015281878144  & 1.3 & 0.9999995 &  Star  \\ 
68011  &  J010542-741907  &  01:05:41.75  &  -74:19:07.0  &  Gaia DR3 4684798357652468736  & - & 0.998 &  RGB*\_Candidate  \\ 
2442  &  J011110-714227  &  01:11:09.81  &  -71:42:26.8  &  Gaia DR3 4687542940583720960  & - & - &  YSO\_Candidate  \\ 
37129  &  J011201-732043  &  01:12:01.39  &  -73:20:43.2  &  Gaia DR3 4687161311240297984  & - & 0.99 &  YSO\_Candidate  \\ 
32548  &  J011244-714040  &  01:12:44.27  &  -71:40:39.7  &  Gaia DR3 4687636295946896512  & 6.9 & 0.993 &  AGN  \\ 
46243  &  J011251-722231  &  01:12:50.61  &  -72:22:30.7  &  Gaia DR3 4687452166424568064  & 1.41 & 0.999991 &  RGB*\_Candidate  \\ 
41292  &  J011322-724520  &  01:13:21.92  &  -72:45:20.4  &  Gaia DR3 4687241365113885440  & 20.5 & 0.9997 &  Star  \\ 
14116  &  J011517-731143  &  01:15:16.56  &  -73:11:43.2  &  Gaia DR3 4687166877510636032  & 31.1 & - &  Star  \\ 
101882  &  J011539-714844  &  01:15:39.01  &  -71:48:44.3  &  Gaia DR3 4687617780347172736  & 0.91 & 0.0 &  RRLyr  \\ 
108120  &  J011705-722844  &  01:17:04.72  &  -72:28:44.2  &  Gaia DR3 4687350732164591104  & 6.54 & 0.99991 &  Star  \\ 
73060  &  J011710-702150  &  01:17:09.72  &  -70:21:49.7  &  Gaia DR3 4690959294964458880  & 33.2 & 0.9998 &  Star  \\ 
30106  &  J012107-733931  &  01:21:06.81  &  -73:39:31.1  &  Gaia DR3 4686435251294836352  & 1.66 & 0.9999998 &  Star  \\ 
28304  &  J012508-734613  &  01:25:08.26  &  -73:46:13.2  &  Gaia DR3 4686231467979348608  & 4.33 & 0.9993 &  Star  \\ 
74414  &  J012711-701022  &  01:27:10.58  &  -70:10:22.5  &  Gaia DR3 4691120446431145088  & 10.3 & 0.999991 &  Cepheid  \\ 
43969  &  J012956-722554  &  01:29:56.49  &  -72:25:53.7  &  Gaia DR3 4686558022933497088  & - & - &  Star  \\ 
96782  &  J013150-725500  &  01:31:49.93  &  -72:55:00.4  &  Gaia DR3 4686483324862269312  & - & 0.0 &  RGB*\_Candidate  \\ 
616  &  J013607-742822  &  01:36:06.71  &  -74:28:22.5  &  Gaia DR3 4638111788265983488  & 1.28 & 0.0 &  RGB*\_Candidate  \\ 
82158  &  J002006-715408  &  00:20:05.72  &  -71:54:08.5  &  Gaia DR3 4689823980486679168  & 5.94 & 0.99998 & - \\ 
14059  &  J002050-744608  &  00:20:49.58  &  -74:46:07.8  &  Gaia DR3 4685365946168078336  & 7.36 & 0.999994 & - \\ 
44915  &  J002120-721558  &  00:21:19.96  &  -72:15:57.7  &  Gaia DR3 4689601157584333696  & 6.22 & 0.99999 & - \\ 
48471  &  J002214-720012  &  00:22:14.39  &  -72:00:11.7  &  Gaia DR3 4689830508848785920  & 5.64 & 0.999997 & - \\ 
85123  &  J002227-715439  &  00:22:26.84  &  -71:54:38.5  &  Gaia DR3 4689832020676672512  & 6.15 & 0.99997 & - \\ 
48777  &  J002248-715902  &  00:22:47.55  &  -71:59:02.0  &  Gaia DR3 4689643012055881856  & 5.27 & 0.99999 & - \\ 
47358  &  J002300-720552  &  00:23:00.06  &  -72:05:52.1  &  Gaia DR3 4689638339132103552  & 6.29 & 0.9999 & - \\ 
47910  &  J002308-720329  &  00:23:07.91  &  -72:03:29.1  &  Gaia DR3 4689638987686114816  & 6.98 & 0.9999991 & - \\ 
45764  &  J002308-721316  &  00:23:08.03  &  -72:13:15.7  &  Gaia DR3 4689624251636760448  & 5.61 & 0.99999 & - \\ 
92483  &  J002310-745944  &  00:23:10.25  &  -74:59:44.2  &  Gaia DR3 4685305537452065792  & 5.66 & 0.99998 & - \\ 
52180  &  J002321-721755  &  00:23:20.94  &  -72:17:54.7  &  Gaia DR3 4689620295995916160  & 5.98 & 0.99998 & - \\ 
45854  &  J002327-721306  &  00:23:26.92  &  -72:13:06.3  &  Gaia DR3 4689624457795419776  & 6.41 & 0.99998 & - \\ 
45048  &  J002335-721658  &  00:23:34.73  &  -72:16:58.1  &  Gaia DR3 4689620330355662592  & 5.32 & 0.99999 & - \\ 
54660  &  J002340-721133  &  00:23:40.12  &  -72:11:33.0  &  Gaia DR3 4689624762757864576  & 5.98 & 0.9996 & - \\ 
46466  &  J002402-721046  &  00:24:01.85  &  -72:10:46.1  &  Gaia DR3 4689624801382291712  & 6.07 & 0.99998 & - \\ 
49654  &  J002427-715601  &  00:24:26.82  &  -71:56:00.9  &  Gaia DR3 4689644828840037504  & 6.94 & 0.999995 & - \\ 
50320  &  J002442-715311  &  00:24:41.95  &  -71:53:11.4  &  Gaia DR3 4689645520316370048  & 5.12 & 0.99997 & - \\ 
97788  &  J002458-715846  &  00:24:57.84  &  -71:58:46.1  &  Gaia DR3 4689641117988195200  & 5.93 & 0.999994 & - \\ 
45609  &  J002510-721516  &  00:25:10.40  &  -72:15:15.6  &  Gaia DR3 4689575220277040128  & 5.35 & 0.999994 & - \\ 
47717  &  J002512-720548  &  00:25:12.30  &  -72:05:48.5  &  Gaia DR3 4689626927404570240  & 6.75 & 0.9994 & - \\ 
48102  &  J002526-720407  &  00:25:26.50  &  -72:04:07.2  &  Gaia DR3 4689627855117675392  & 5.11 & 0.99999 & - \\ 
96854  &  J002555-720801  &  00:25:54.94  &  -72:08:01.4  &  Gaia DR3 4689629366946486016  & 7.35 & 0.999996 & - \\ 
89969  &  J002616-721913  &  00:26:15.61  &  -72:19:13.0  &  Gaia DR3 4689576590373076096  & 6.44 & 0.99998 & - \\ 
100201  &  J002626-715711  &  00:26:26.21  &  -71:57:10.6  &  Gaia DR3 4689646241872963328  & 5.55 & 0.99994 & - \\ 
56364  &  J002715-712948  &  00:27:14.60  &  -71:29:47.9  &  Gaia DR3 4689859577177622016  & 5.96 & 0.99998 & - \\ 
56668  &  J002741-744049  &  00:27:41.09  &  -74:40:48.9  &  Gaia DR3 4685345467763983104  & 16.5 & 0.99998 & - \\ 
3533  &  J003115-712733  &  00:31:15.32  &  -71:27:33.0  &  Gaia DR3 4690220629314974080  & 9.17 & 0.99994 & - \\ 
56514  &  J003329-713246  &  00:33:29.25  &  -71:32:46.1  &  Gaia DR3 4690033750987052800  & 52.0 & 0.99995 & - \\ 
28378  &  J003338-734520  &  00:33:38.20  &  -73:45:19.7  &  Gaia DR3 4688811880046094464  & 12.9 & 0.0 & - \\ 
43203  &  J003400-701428  &  00:34:00.04  &  -70:14:27.8  &  Gaia DR3 4702375253610789504  & 5.6 & 0.997 & - \\ 
39063  &  J003523-725158  &  00:35:22.75  &  -72:51:58.2  &  Gaia DR3 4689100918454849536  & 6.53 & 0.999 & - \\ 
35943  &  J003947-730935  &  00:39:46.87  &  -73:09:34.6  &  Gaia DR3 4688867753275963904  & 10.7 & - & - \\ 
94389  &  J004035-744624  &  00:40:34.58  &  -74:46:24.0  &  Gaia DR3 4685464176365992064  & 8.16 & 0.9991 & - \\ 
21364  &  J004243-742240  &  00:42:42.53  &  -74:22:40.4  &  Gaia DR3 4685555710710807680  & 8.94 & 0.999992 & - \\ 
107369  &  J004322-740801  &  00:43:22.39  &  -74:08:01.0  &  Gaia DR3 4685749877647472896  & 9.42 & 0.9998 & - \\ 
40617  &  J004353-724751  &  00:43:52.83  &  -72:47:51.3  &  Gaia DR3 4688926366745349248  & 5.45 & 0.995 & - \\ 
38060  &  J004417-733709  &  00:44:16.97  &  -73:37:09.1  &  Gaia DR3 4685823579241206272  & 7.17 & 0.992 & - \\ 
29124  &  J004627-734621  &  00:46:27.07  &  -73:46:20.9  &  Gaia DR3 4685776265879398656  & 10.9 & 0.9999 & - \\ 
35036  &  J004733-731701  &  00:47:33.22  &  -73:17:01.0  &  Gaia DR3 4685942708820468224  & 12.8 & 0.998 & - \\ 
49167  &  J004752-732455  &  00:47:52.47  &  -73:24:54.9  &  Gaia DR3 4685926422305317504  & 10.1 & 0.9998 & - \\ 
105480  &  J004757-715314  &  00:47:57.28  &  -71:53:14.2  &  Gaia DR3 4689263298283177088  & 8.6 & 0.99999 & - \\ 
87528  &  J004851-734127  &  00:48:50.69  &  -73:41:26.7  &  Gaia DR3 4685860481601577344  & 7.86 & 0.9999993 & - \\ 
50710  &  J004916-720218  &  00:49:16.22  &  -72:02:17.7  &  Gaia DR3 4689243305204078592  & 5.78 & 0.998 & - \\ 
3083  &  J004950-724256  &  00:49:50.00  &  -72:42:55.8  &  Gaia DR3 4688977562777617792  & 7.68 & 0.9996 & - \\ 
32061  &  J004954-733316  &  00:49:54.42  &  -73:33:15.7  &  Gaia DR3 4685874053772462720  & 23.7 & 0.97 & - \\ 
36149  &  J005027-731110  &  00:50:26.91  &  -73:11:10.1  &  Gaia DR3 4685933397271717760  & 8.55 & 0.998 & - \\ 
50623  &  J005033-720255  &  00:50:32.96  &  -72:02:55.3  &  Gaia DR3 4689243614440935040  & 6.61 & 0.99997 & - \\ 
9503  &  J005319-732145  &  00:53:19.01  &  -73:21:44.6  &  Gaia DR3 4685882849826495616  & 5.14 & 0.994 & - \\ 
34766  &  J005321-731916  &  00:53:20.92  &  -73:19:16.3  &  Gaia DR3 4685883232049431936  & 17.0 & - & - \\ 
21946  &  J005445-745554  &  00:54:45.49  &  -74:55:53.9  &  Gaia DR3 4684753312040026112  & 38.8 & 0.996 & - \\ 
95834  &  J005447-732341  &  00:54:47.45  &  -73:23:41.3  &  Gaia DR3 4685871721572256128  & 6.65 & 0.998 & - \\ 
67983  &  J005448-740122  &  00:54:47.54  &  -74:01:22.2  &  Gaia DR3 4685605914599331200  & 20.8 & - & - \\ 
94547  &  J005457-733509  &  00:54:57.20  &  -73:35:08.6  &  Gaia DR3 4685677859622440576  & 5.78 & 0.997 & - \\ 
3340  &  J005513-733800  &  00:55:12.87  &  -73:38:00.3  &  Gaia DR3 4685676798744979584  & 6.07 & 0.9998 & - \\ 
86301  &  J005516-715240  &  00:55:16.32  &  -71:52:40.2  &  Gaia DR3 4689087445145894400  & 7.54 & 0.99996 & - \\ 
37152  &  J005621-730647  &  00:56:20.66  &  -73:06:46.6  &  Gaia DR3 4685912815770474368  & 13.0 & 0.996 & - \\ 
33437  &  J005727-732727  &  00:57:26.92  &  -73:27:26.7  &  Gaia DR3 4685702602915240320  & 5.57 & 0.9997 & - \\ 
43267  &  J005759-723741  &  00:57:59.21  &  -72:37:40.8  &  Gaia DR3 4685988613398832000  & 21.2 & 0.99998 & - \\ 
16681  &  J005815-744629  &  00:58:14.85  &  -74:46:29.0  &  Gaia DR3 4684760561944723456  & 29.4 & 0.99992 & - \\ 
35228  &  J005858-731720  &  00:58:57.64  &  -73:17:19.9  &  Gaia DR3 4685893093274871808  & 7.77 & 0.995 & - \\ 
90710  &  J005951-724133  &  00:59:51.26  &  -72:41:33.5  &  Gaia DR3 4685976037726446848  & 6.93 & 0.9999995 & - \\ 
99522  &  J010014-724808  &  01:00:13.93  &  -72:48:08.1  &  Gaia DR3 4685971429279805952  & 6.38 & 0.999999 & - \\ 
30877  &  J010108-715526  &  01:01:08.43  &  -71:55:25.6  &  Gaia DR3 4690524472511001088  & 5.33 & 0.996 & - \\ 
101254  &  J010125-705441  &  01:01:25.45  &  -70:54:40.7  &  Gaia DR3 4690862366142213504  & 7.01 & 0.9999 & - \\ 
41878  &  J010150-724358  &  01:01:49.60  &  -72:43:58.3  &  Gaia DR3 4687426362243482880  & 5.66 & 0.99999 & - \\ 
66888  &  J010233-705451  &  01:02:33.30  &  -70:54:50.6  &  Gaia DR3 4690839074535209088  & 6.92 & 0.999994 & - \\ 
31709  &  J010246-733545  &  01:02:45.78  &  -73:35:45.1  &  Gaia DR3 4685642572128613888  & 8.17 & 0.9998 & - \\ 
67065  &  J010304-705402  &  01:03:03.52  &  -70:54:01.7  &  Gaia DR3 4690838937096176256  & 8.45 & 0.9999 & - \\ 
103124  &  J010310-705235  &  01:03:09.68  &  -70:52:35.2  &  Gaia DR3 4690839589930865664  & 15.0 & - & - \\ 
33424  &  J010338-732726  &  01:03:38.34  &  -73:27:25.8  &  Gaia DR3 4685691573434514176  & 10.2 & 0.995 & - \\ 
46720  &  J010549-722141  &  01:05:49.46  &  -72:21:40.6  &  Gaia DR3 4687488587757074944  & 7.37 & 0.9999995 & - \\ 
90784  &  J010619-760151  &  01:06:19.41  &  -76:01:51.2  &  Gaia DR3 4636420975604052096  & 9.37 & 0.99997 & - \\ 
50096  &  J010631-714838  &  01:06:31.12  &  -71:48:38.5  &  Gaia DR3 4690540282257021440  & 10.9 & 0.99993 & - \\ 
92488  &  J010638-721544  &  01:06:37.51  &  -72:15:44.3  &  Gaia DR3 4687490340103198208  & 8.29 & 0.99995 & - \\ 
103644  &  J010711-753224  &  01:07:11.07  &  -75:32:24.1  &  Gaia DR3 4684485198699244672  & 30.1 & 0.9999 & - \\ 
98866  &  J010746-704641  &  01:07:45.88  &  -70:46:41.0  &  Gaia DR3 4690832683625105152  & 12.4 & 0.99997 & - \\ 
75076  &  J011249-701317  &  01:12:48.53  &  -70:13:17.0  &  Gaia DR3 4690956138162512256  & 20.5 & 0.99996 & - \\ 
103660  &  J011433-722356  &  01:14:33.49  &  -72:23:56.4  &  Gaia DR3 4687449623791632768  & 5.14 & 0.9997 & - \\ 
75486  &  J011642-700957  &  01:16:41.77  &  -70:09:56.7  &  Gaia DR3 4690971045995196672  & 8.48 & 0.9999 & - \\ 
105061  &  J011736-695732  &  01:17:35.86  &  -69:57:32.0  &  Gaia DR3 4690989467109599872  & 9.13 & 0.99997 & - \\ 
54927  &  J012221-714122  &  01:22:20.77  &  -71:41:22.2  &  Gaia DR3 4687587337618874240  & 18.4 & 0.99998 & - \\ 
102248  &  J012231-721332  &  01:22:31.07  &  -72:13:31.9  &  Gaia DR3 4687372447516963968  & 8.25 & 0.99997 & - \\ 
59285  &  J012313-712323  &  01:23:13.26  &  -71:23:23.0  &  Gaia DR3 4687611660018743040  & 5.13 & 0.99999 & - \\ 
27921  &  J012740-734651  &  01:27:39.77  &  -73:46:50.6  &  Gaia DR3 4686223290360321664  & 36.2 & 0.99999 & - \\ 
37203  &  J013527-725507  &  01:35:27.13  &  -72:55:07.5  &  Gaia DR3 4686843586718702464  & 24.4 & 0.999993 & - \\ 
101795  &  J013657-701539  &  01:36:56.66  &  -70:15:39.0  &  Gaia DR3 4688184166269149696  & 18.9 & - & - \\ 
69849  &  J014028-702341  &  01:40:27.60  &  -70:23:41.0  &  Gaia DR3 4688123860632580352  & 10.1 & 0.9999 & - \\ 
45839  &  J002314-721259  &  00:23:13.74  &  -72:12:59.5  &  0.0  & - & - &  RGB*\_Candidate  \\ 
42977  &  J002346-722628  &  00:23:46.03  &  -72:26:27.7  &  0.0  & - & - &  Star  \\ 
82932  &  J002449-720420  &  00:24:48.89  &  -72:04:19.7  &  0.0  & - & - &  Star  \\ 
34163  &  J002608-731253  &  00:26:07.85  &  -73:12:53.0  &  0.0  & - & - &  RGB*\_Candidate  \\ 
47612  &  J002723-720747  &  00:27:22.97  &  -72:07:46.9  &  0.0  & - & - &  RGB*\_Candidate  \\ 
86652  &  J002845-742319  &  00:28:44.66  &  -74:23:19.0  &  0.0  & - & - &  Star  \\ 
90970  &  J002957-732631  &  00:29:57.41  &  -73:26:30.7  &  0.0  & - & - &  RGB*\_Candidate  \\ 
25590  &  J003204-735836  &  00:32:04.40  &  -73:58:36.1  &  0.0  & - & - &  RGB*\_Candidate  \\ 
24070  &  J003546-740737  &  00:35:45.50  &  -74:07:37.0  &  0.0  & - & - &  RGB*\_Candidate  \\ 
91676  &  J003611-730447  &  00:36:11.19  &  -73:04:47.5  &  0.0  & - & - &  Star  \\ 
10091  &  J003637-703902  &  00:36:36.97  &  -70:39:01.9  &  0.0  & - & - &  RGB*\_Candidate  \\ 
33530  &  J003707-725652  &  00:37:07.22  &  -72:56:52.4  &  0.0  & - & - &  RGB*\_Candidate  \\ 
79608  &  J003947-730434  &  00:39:46.72  &  -73:04:34.5  &  0.0  & - & - &  Star  \\ 
36418  &  J004044-730703  &  00:40:43.84  &  -73:07:02.9  &  0.0  & - & - &  RGB*\_Candidate  \\ 
90131  &  J004058-733258  &  00:40:58.03  &  -73:32:57.5  &  0.0  & - & - &  RGB*\_Candidate  \\ 
86989  &  J004423-733343  &  00:44:23.32  &  -73:33:43.1  &  0.0  & - & - &  YSO\_Candidate  \\ 
101160  &  J004439-722832  &  00:44:39.30  &  -72:28:31.7  &  0.0  & - & - &  RGB*\_Candidate  \\ 
4230  &  J004440-731803  &  00:44:39.67  &  -73:18:03.4  &  0.0  & - & - &  RGB*\_Candidate  \\ 
65251  &  J004548-735331  &  00:45:47.66  &  -73:53:31.2  &  0.0  & - & - &  YSO\_Candidate  \\ 
93554  &  J004549-731956  &  00:45:48.52  &  -73:19:56.0  &  0.0  & - & - &  RRLyr  \\ 
41586  &  J004750-724412  &  00:47:49.87  &  -72:44:11.7  &  0.0  & - & - &  RGB*\_Candidate  \\ 
105967  &  J004751-714459  &  00:47:50.62  &  -71:44:59.5  &  0.0  & - & - &  Star  \\ 
94467  &  J004832-720536  &  00:48:31.93  &  -72:05:35.9  &  0.0  & - & - &  YSO\_Candidate  \\ 
48296  &  J004859-720312  &  00:48:59.30  &  -72:03:12.1  &  0.0  & - & - &  RGB*\_Candidate  \\ 
101293  &  J004902-731110  &  00:49:01.74  &  -73:11:10.1  &  0.0  & - & - &  YSO  \\ 
32390  &  J004907-733137  &  00:49:06.71  &  -73:31:36.6  &  0.0  & - & - &  Star  \\ 
30605  &  J004950-734011  &  00:49:49.93  &  -73:40:11.2  &  0.0  & - & - &  YSO\_Candidate  \\ 
103523  &  J005023-743251  &  00:50:23.39  &  -74:32:50.8  &  0.0  & - & - &  RGB*\_Candidate  \\ 
95386  &  J005040-711851  &  00:50:40.49  &  -71:18:51.4  &  0.0  & - & - &  RRLyr  \\ 
53790  &  J005046-714938  &  00:50:45.74  &  -71:49:38.2  &  0.0  & - & - &  RGB*\_Candidate  \\ 
29712  &  J005141-734440  &  00:51:41.27  &  -73:44:39.9  &  0.0  & - & - &  RGB*\_Candidate  \\ 
101604  &  J005210-732105  &  00:52:09.82  &  -73:21:05.4  &  0.0  & - & - &  YSO\_Candidate  \\ 
60826  &  J005221-740417  &  00:52:20.63  &  -74:04:17.1  &  0.0  & - & - &  RGB*\_Candidate  \\ 
37248  &  J005310-730602  &  00:53:10.29  &  -73:06:01.8  &  0.0  & - & - &  RGB*\_Candidate  \\ 
104742  &  J005328-723024  &  00:53:27.61  &  -72:30:23.9  &  0.0  & - & - &  RGB*\_Candidate  \\ 
87988  &  J005328-733339  &  00:53:27.97  &  -73:33:38.9  &  0.0  & - & - &  Star  \\ 
40774  &  J005330-715308  &  00:53:29.63  &  -71:53:07.6  &  0.0  & - & - &  RGB*\_Candidate  \\ 
96813  &  J005411-732423  &  00:54:11.13  &  -73:24:22.7  &  0.0  & - & - &  RGB*\_Candidate  \\ 
56931  &  J005425-713747  &  00:54:24.56  &  -71:37:47.2  &  0.0  & - & - &  RGB*\_Candidate  \\ 
94103  &  J005427-724507  &  00:54:26.82  &  -72:45:07.1  &  0.0  & - & - &  RGB*\_Candidate  \\ 
47442  &  J005440-721823  &  00:54:39.95  &  -72:18:23.5  &  0.0  & - & - &  RRLyr  \\ 
68828  &  J005553-725230  &  00:55:53.08  &  -72:52:29.9  &  0.0  & - & - &  YSO\_Candidate  \\ 
5192  &  J005714-732858  &  00:57:13.59  &  -73:28:58.2  &  0.0  & - & - &  RGB*\_Candidate  \\ 
49220  &  J005730-721009  &  00:57:30.16  &  -72:10:08.8  &  0.0  & - & - &  Star  \\ 
49503  &  J005810-720841  &  00:58:10.01  &  -72:08:40.9  &  0.0  & - & - &  YSO\_Candidate  \\ 
49576  &  J005830-720841  &  00:58:30.32  &  -72:08:41.2  &  0.0  & - & - &  YSO  \\ 
12404  &  J005902-722950  &  00:59:02.15  &  -72:29:50.0  &  0.0  & - & - &  YSO\_Candidate  \\ 
3413  &  J005924-741959  &  00:59:24.04  &  -74:19:59.4  &  0.0  & - & - &  RGB*\_Candidate  \\ 
44253  &  J005932-720454  &  00:59:32.31  &  -72:04:53.7  &  0.0  & - & - &  YSO\_Candidate  \\ 
65781  &  J005937-721423  &  00:59:37.06  &  -72:14:23.0  &  0.0  & - & - &  YSO  \\ 
66130  &  J005952-721540  &  00:59:52.26  &  -72:15:40.4  &  0.0  & - & - &  YSO  \\ 
45505  &  J005955-722716  &  00:59:55.24  &  -72:27:16.1  &  0.0  & - & - &  RGB*\_Candidate  \\ 
61566  &  J010015-721629  &  01:00:15.41  &  -72:16:28.6  &  0.0  & - & - &  YSO  \\ 
95061  &  J010046-724633  &  01:00:46.35  &  -72:46:32.5  &  0.0  & - & - &  RGB*\_Candidate  \\ 
89571  &  J010050-723500  &  01:00:49.76  &  -72:35:00.3  &  0.0  & - & - &  Star  \\ 
509  &  J010109-725024  &  01:01:09.07  &  -72:50:24.0  &  0.0  & - & - &  RGB*\_Candidate  \\ 
94788  &  J010113-733321  &  01:01:13.44  &  -73:33:20.9  &  0.0  & - & - &  RGB*\_Candidate  \\ 
26288  &  J010248-740152  &  01:02:48.00  &  -74:01:51.8  &  0.0  & - & - &  Star  \\ 
2102  &  J010253-705050  &  01:02:53.02  &  -70:50:50.1  &  0.0  & - & - &  Star  \\ 
35102  &  J010313-731751  &  01:03:12.99  &  -73:17:51.2  &  0.0  & - & - &  RGB*\_Candidate  \\ 
38342  &  J010447-715526  &  01:04:46.69  &  -71:55:25.7  &  0.0  & - & - &  YSO\_Candidate  \\ 
48843  &  J010838-721122  &  01:08:38.30  &  -72:11:21.6  &  0.0  & - & - &  RGB*\_Candidate  \\ 
56769  &  J010940-713749  &  01:09:39.52  &  -71:37:49.4  &  0.0  & - & - &  RGB*\_Candidate  \\ 
43720  &  J011125-723414  &  01:11:24.92  &  -72:34:14.1  &  0.0  & - & - &  RGB*\_Candidate  \\ 
57385  &  J011144-713454  &  01:11:44.11  &  -71:34:54.5  &  0.0  & - & - &  RGB*\_Candidate  \\ 
45641  &  J011245-722511  &  01:12:45.08  &  -72:25:11.1  &  0.0  & - & - &  RGB*\_Candidate  \\ 
85335  &  J012454-733833  &  01:24:54.43  &  -73:38:33.1  &  0.0  & - & - &  Star  \\ 
33160  &  J012914-731342  &  01:29:13.59  &  -73:13:42.1  &  0.0  & - & - &  RRLyr  \\ 
29946  &  J012941-733625  &  01:29:41.28  &  -73:36:25.0  &  0.0  & - & - &  YSO\_Candidate  \\ 
39125  &  J013001-732409  &  01:30:00.96  &  -73:24:09.0  &  0.0  & - & - &  Star  \\ 
42410  &  J013919-722654  &  01:39:18.69  &  -72:26:54.4  &  0.0  & - & - &  Star  \\ 
\end{tabular}
\end{table}

